Singular Layer Physics-Informed Neural Network Method for Convection-Dominated Boundary Layer Problems in Two Dimensions

This research explores neural network-based numerical approximation of two-dimensional convection-dominated singularly perturbed problems on square, circular, and elliptic domains. Singularly perturbed boundary value problems pose significant challenges due to sharp boundary layers in their solutions. Additionally, the characteristic points of these domains give rise to degenerate boundary layer problems. The stiffness of these problems, caused by sharp singular layers, can lead to substantial computational errors if not properly addressed. Conventional neural network-based approaches often fail to capture these sharp transitions accurately, highlighting a critical flaw in machine learning methods. To address these issues, we conduct a thorough boundary layer analysis to enhance our understanding of sharp transitions within the boundary layers, guiding the application of numerical methods. Specifically, we employ physics-informed neural networks (PINNs) to better handle these boundary layer problems. However, PINNs may struggle with rapidly varying singularly perturbed solutions in small domain regions, leading to inaccurate or unstable results. To overcome this limitation, we introduce a semi-analytic method that augments PINNs with singular layers or corrector functions. Our numerical experiments demonstrate significant improvements in both accuracy and stability, showcasing the effectiveness of our proposed approach.

==> Boundary_layer_analysis.tex <==


    

{\color{red}
\section{Boundary Layer Analysis}
In this section, we address singularly perturbed problems and perform boundary layer analysis using the corrector method for various domain scenarios. The analysis varies based on the shape of the domains, as the boundary layer behavior differs in each case.


Let's consider the following partial differential equation: 
\begin{equation}\label{original pde}
\left\{
\begin{aligned}
L_\varepsilon u^\varepsilon &:= -\varepsilon \Delta u^\varepsilon - u^\varepsilon_y = f(x, y) \text{ in } D, \\
u^\varepsilon &= 0 \text{ on } \partial D,
\end{aligned}
\right.
\end{equation}
where \(0 < \varepsilon \ll 1\). The domain \(D\) is an ellipse defined as \(\ D = \{(x, y) \mid \frac{x^2}{A^{2}} + \frac{y^{2}}{B^{2}} < 1\}\) where $A=a\cosh R$, $B=a\sinh R$,  and the function \(f\) is assumed to be as smooth as needed.
For the domain \(D\), which can vary in shape (square or circle), we focus particularly on the ellipse with its major axis parallel to the \(x\)-axis. 
The limit problem (i.e., when \(\varepsilon = 0\)) is defined by
\begin{equation}\label{limit equation}
\left\{
\begin{aligned}
-u^0_y &= f(x, y) \text{ in } D, \\
u^0 &= 0 \text{ on } \Gamma_u,
\end{aligned}
\right.
\end{equation}
where \(\Gamma_u = \{(x, y) \mid \frac{x^2}{A^{2}} + \frac{y^{2}}{B^{2}} = 1, y > 0\}\). The explicit solution of equation (\ref{limit equation}) is
\begin{equation}\label{limit solution}
u^0(x, y) = \int^{C_u(x)}_{y} f(x, s) ds, \quad (x, y) \in D,
\end{equation}
which \(C_u(x) = B\sqrt{1 - \frac{x^{2}}{A^{2}}}\) is upper halves of the ellipse. We define boundary fitted coordinate for an elliptic coordinate system such that 
\begin{equation}
x = a \cosh (R-\eta) \cos \tau, \quad y = a \sinh (R-\eta) \sin \tau,
\end{equation}
where the elliptic domain \( D \) changed to \( D^* = \{ (\eta, \tau) \in (0, R) \times (0, 2\pi) \}\), and \( R \) is the maximal radial extent.
\begin{comment}
    where \( r \) be the radial distance from the center to a point within the domain \( D \), and let \( \xi \) be the angular coordinate, representing the angle relative to the positive \( x \)-axis in our elliptic coordinate system. 

We map the elliptic domain \( D^* = \{ (r, \xi) \in (0, R) \times (0, 2\pi) \}\), where \( R \) is the maximal radial extent.
\end{comment}
We also define the domain \(D^*_{R/2}\) as \(D^*_{R/2} = \{ (\eta, \tau) \in D^* : r \leq \frac{R}{2} \}\).
In these coordinates, the transformed differential operator for equation (\ref{original pde}) is given by
\begin{equation}\label{Transforemd pde}
\begin{aligned}
L_\epsilon u^\epsilon &= -\epsilon \Delta u^\epsilon - u^\epsilon_y \\
&= \frac{1}{H} \left(-\epsilon (v^{\epsilon}_{\eta \eta} + v^{\epsilon}_{\tau \tau}) + (a \cosh (R-\eta) \sin \tau) v^{\epsilon}_{\eta} - (a \sinh (R-\eta) \cos \tau) v^{\epsilon}_{\tau} \right),
\end{aligned}
\end{equation}
where \(H = (a\sinh (R-\eta) \cos \tau)^{2} + (a \cosh (R-\eta) \sin \tau)^{2}\).
Considering the stretched variable \(\tilde{\eta} = \frac{\eta}{\epsilon}\), we change (\ref{Transforemd pde}) to:
\begin{equation}\label{enriched transforemd pde}
\begin{aligned}
L_\epsilon u^\epsilon &= -\epsilon \Delta u^\epsilon - u^\epsilon_y \\
&= \frac{1}{H} \left(-\frac{1}{\epsilon} v^{\epsilon}_{\tilde{\eta}\tilde{\eta}} -\epsilon v^{\epsilon}_{\tau \tau} + \frac{1}{\epsilon}(a \cosh (R- \tilde{\eta}) \sin \tau) v^{\epsilon}_{\tilde{\eta}} - (a \sinh (R-\tilde{\eta}) \cos \tau) v^{\epsilon}_{\tau} \right).
\end{aligned}
\end{equation}


%Full error analysis and further lemmas ensure the robustness of our results, aiming to approximate solutions efficiently and accurately.

To get rid of the leading terms of (\ref{enriched transforemd pde}) and to ensure matching at the boundary,
we are led to the following equation for the first corrector  \(\theta^0\):
\begin{equation}\label{corrector equation}
\left\{
\begin{aligned}
-\frac{\partial^2 \theta^{\epsilon}}{\partial \tilde{\eta}^2} + a\cosh( R-\epsilon \tilde{\eta}) \sin \tau \frac{\partial \theta^{\epsilon}}{\partial \tilde{\eta}} &= 0, & \text{for } 0 < \tilde{\eta} < \infty, \pi < \tau < 2\pi, \\
\theta^{\epsilon} &= -u^0 (a \cosh R \cos \tau, a\sinh R \sin \tau) & \text{at } \tilde{\eta} = 0, \\
\theta^{\epsilon} &\rightarrow 0 & \text{as } \tilde{\eta} \rightarrow \infty.
\end{aligned}
\right.
\end{equation}
Instead of directly finding the explicit solution in \eqref{corrector equation}, we look for an approximation of the solution in \eqref{Approximated corrector equation} using the following form:
\begin{equation}\label{Approximated corrector equation}
\left\{
\begin{aligned}
-\frac{\partial^2 \theta^0}{\partial \tilde{\eta}^2} + a\cosh R \sin \tau \frac{\partial \theta^0}{\partial \tilde{\eta}} &= 0, & \text{for } 0 < \tilde{\eta} < \infty, \pi < \tau < 2\pi, \\
\theta^0 &= -u^0 (a \cosh R \cos \tau, a\sinh R \sin \tau) & \text{at } \tilde{\eta} = 0, \\
\theta^0 &\rightarrow 0 & \text{as } \tilde{\eta} \rightarrow \infty.
\end{aligned}
\right.
\end{equation}
An explicit solution is directly obtained by:
\begin{equation}
\theta^0 = -u^0 (a \cosh R \cos \tau, a \sinh R \sin \tau) \exp \left( \frac{R^x \sin \tau }{\epsilon}\eta \right) \chi_{[\pi, 2\pi)}(\tau),
\end{equation}
where \(\chi_A\) is the characteristic function of the set \(A\) and \(R^x = a \cosh R\). Using a cut-off function we write an approximate form of \(\theta^0\):
\begin{equation}\label{delta corrector}
\bar{\theta}^0 = -u^0 (a \cosh R \cos \tau, a \sinh R \sin \tau) \exp \left( \frac{R^x \sin \tau }{\epsilon}\eta \right) \delta(\eta) \chi_{[\pi, 2\pi)}(\tau),
\end{equation}
where \(\delta(\eta)\) is a smooth cut-off function such that \(\delta(\eta) = 1\) for \(\eta \in [0, R/4]\) and \(= 0\) for \(\eta \in [R/2, R]\).

Since \(\theta^0\) vanishes \(u^0\) like at \(\tau = \pi, 2\pi\), \(\theta^0\) is continuous and piecewise smooth on \(\overline{D}\), and thus we conclude that \(\theta^0, \bar{\theta}^0 \in H^1(D)\). 
We then obtain that 
\begin{equation}
u^0 + \bar{\theta}^0 \in H^1_0(D).
\end{equation}
{\color{blue}
Note that if \( f = f(x, y) \) does not vanish at the characteristic points \((\pm a\cosh R, 0)\), \( f(x, y) \) is incompatible in the sense that singularities of the derivatives of \( u^0 \) will occur at these points (see \cite{JUNG201188}). More general singularity and compatibility issues can be handled by considering more general compatibility conditions.} Furthermore, compatibility plays a crucial role in ensuring the boundedness of functions and in the applicability of convergence theorems.



\begin{comment}
\textbf{Lemma 3.1.} The boundary layer approximated correctors \(\theta^j\) are explicitly given by:
\[
\theta^j = P^j (\xi, \tilde{r}) \exp(R^{x}(\sin \xi) \overline{r}) \chi_{[\pi,2\pi)}(\xi), \quad j \geq 0,
\tag{3.11}
\]
where
\[
P^j (\xi, \tilde{r}) = \sum_{i=0}^{j} \sum_{k=0}^{2j-2i} a_{i,3j-3i-k}(\xi) \tilde{r}^k,
\tag{3.12}
\]
\[
a_{i,q}(\xi) = \sum_{\substack{m+r \leq q \\ m,r \geq 0}} \frac{c_{m,r}} {\sin^m \xi}\frac{d^r v^i (\xi)} {d\xi^r},
\tag{3.13}
\]
and \(v^j (\xi) = -u^j(a\cosh R\cos \xi, a\sinh R\sin \xi)\). Here the coefficients \(c_{m,r} = c_{m,r}(\xi) \in C^\infty([0, 2\pi])\) may be different at different occurrences.
\end{comment}






\begin{comment}
More general singularity and compatibility issues can be handled by considering more general compatibility conditions of the form (see \cite{21}):
\begin{equation}
\frac{\partial^{p1+p2} f}{\partial x^{p1} \partial y^{p2}} = 0 \text{ at } (\pm 1, 0) \text{ for } 0 \leq 2p1 + p2 \leq 2 + 3n, \text{ and } p1, p2 \geq 0.
\end{equation} 
\end{comment}






.

\begin{comment}
    Then the functions
\[
\frac{1}{(\sin \xi)^{q-r}} \frac{d^r v^i}{d \xi^r}
\]
are bounded for \( \xi \in [\pi, 2\pi] \), \( r = 0, \ldots, q \),
Here \( v^i(\xi) = -u^i(a\cosh R \cos \xi,a\sinh R \sin \xi) \).
\end{comment}







%\begin{lemma}


\noindent\textbf{Lemma 2.1.} We assume that
\begin{equation}
\frac{\partial^{\alpha+\beta} f(x, y)}{\partial x^\alpha \partial y^\beta} = 0 \quad \text{at } (\pm a\cosh R, 0), \quad 0 \leq 2\alpha + \beta \leq \gamma - 1, \quad \gamma \geq 1, \quad \alpha, \beta \geq 0,
\end{equation}
where \( f(x, y) \) belongs to \( C^\gamma(D) \), and \( D \) is the ellipse as in (\ref{original pde}). Then the following function
\begin{equation}
\frac{f(x, C_u(x))}{C^\gamma_u(x)}
\end{equation}
is bounded for all \( x \in (-a\cosh R, a\cosh R) \).










In our analysis, we assume that the following conditions hold:

\begin{equation}\label{general compatibility condition}
\frac{\partial^{p_{1}+p_{2}} f}{\partial x^{p_{1}} \partial y^{p_{2}}} = 0 \text{ at } (\pm a\cosh R, 0) \text{ for } 0 \leq 2p_{1} + p_{2} \leq 2 + 3n, \text{ and } p_{1}, p_{2} \geq 0.
\end{equation} 

For experiments and examples, the second compatibility condition, as listed below, was used.

\begin{equation}
\frac{\partial^{p_{1}+p_{2}} f}{\partial x^{p_{1}} \partial y^{p_{2}}} = 0 \quad \text{at} \quad (\pm a\cosh R, 0) \quad \text{for} \quad 0 \leq 2p_{1} + p_{2} \leq 2 , \quad p_{1}, p_{2} \geq 0,
\end{equation}



\noindent \textbf{Lemma 2.2.} There exists a positive constant \( k \) such that, for integers \( l, n, s \geq 0, m = 0, 1, 2 \), and for \( 1 \leq p \leq \infty \),
\begin{equation}
\left| (\sin \tau)^{-l} \left( \frac{\eta}{\varepsilon} \right)^n  \frac{\partial^{s+m} \theta^{0}}{\partial \eta^s \partial \tau^m} \right|_{L_p(D^*)} \leq \kappa \sup_{\tau} |a_{0,h}(\tau)| \varepsilon^{\frac{1}{p}-s},
\end{equation}
where \( h = -s + m + l + n + 1 \), and
\begin{equation}
a_{0,q}(\tau) = \sum_{\substack{m+r \leq q \\ m,r \geq 0}} c_{m,r} \frac{d^r v^0(\tau)}{\sin^m \tau \, d\tau^r},
\end{equation}
\( v^0(\tau) = -u^0(a\cosh R\cos \tau, a\sinh R\sin \tau) \) and the \( c_{m,r} = c_{m,r}(\tau)  \in C^{\infty}([0,2\pi])\), may be different at different occurrences,
If \(q<0 \), then \( a_{0,q}\) is simply in \(C^{\infty}([0,2\pi])\) fuction.
The notation \( a_{0,q} \) follows the same convention as outlined in the \textit{Notation convection} of \cite{JUNG201188}.


%\end{lemma}









\begin{proof}




By using an Inductive approach, for integers \( s \geq 0, m = 0, 1, 2 \), we easily obtain
\begin{equation}
\frac{\partial^{s+m}\theta^0}{\partial \bar{\eta}^{s} \partial \tau^{m}} = \epsilon^{s} \frac{\partial^{s+m}\theta^0}{\partial \eta^{s} \partial \tau^{m}} = a_{0,-s+m}(\tau) \sum_{k=0}^{m} \left( (-\sin \tau)\bar{\eta} \right)^{k} \exp\left( (R^x\sin \tau)\bar{\eta} \right) \chi_{[\pi,2\pi]}(\tau).
\end{equation}
\text{Hence, we observe that}
\begin{equation}
(\sin \tau)^{-l} \bar{\eta}^{n} \frac{\partial^{s+m}\theta^0}{\partial \eta^{s} \partial \tau^{m}} = a_{0,-s+m}(\tau) (\sin \tau)^{-1-l-n} \sum_{k=0}^{m} (-\sin \tau)\left( (-\sin \tau)\bar{\eta} \right)^{k+n} \epsilon^{-s}\exp\left( (R^x\sin \tau)\bar{\eta} \right) \chi_{[\pi,2\pi]}(\tau),
\end{equation}


%\begin{comment}
\begin{equation}
\left| (\sin \tau)^{-l} \bar{\eta}^{n} \frac{\partial^{s+m}\theta^0}{\partial \eta^{s} \partial \tau^{m}} \right|_{L^p(D^*)}
\end{equation}
\begin{equation}
\begin{aligned}
= \left| a_{0,-s+m}(\tau) (\sin \tau)^{-1-l-n} \sum_{k=0}^{m} (-\sin \tau)\left( (-\sin \tau)\bar{\eta} \right)^{k+n} \epsilon^{-s}\exp\left( (R^x\sin \tau)\bar{\eta} \right) \right|_{L^p((0,R) \times (\pi,2\pi))}
\end{aligned}
\end{equation}



\begin{equation}
\leq k \left\{ \sup_{\tau} |a_{0,-s+m+l+n+1}(\tau)| \right\} \left( \int_{\pi}^{2\pi} \int_{0}^{R} |\sum_{k=0}^{m} \left( (-\sin \tau)\bar{\eta} \right)^{k+n}|^{p} (-\sin \tau)^{p}\epsilon^{-ps}\exp\left( (p R^x\sin \tau)\bar{\eta} \right)d\eta d\tau \right)^{\frac{1}{p}}
\end{equation}

\begin{equation}
\leq k \left\{ \sup_{\tau} |a_{0,-s+m+l+n+1}(\tau)| \right\} \left( \int_{\pi}^{2\pi} \int_{0}^{R}  \kappa(-\sin \tau)^{p}\epsilon^{-ps}\exp\left( (p R^x\sin \tau)\bar{\eta} \right)d\eta d\tau \right)^{\frac{1}{p}}
\end{equation}
Using 
\begin{equation}
\int_{\pi}^{2\pi} \int_{0}^{R} (-\sin \tau)^{p} \exp\left( c(R^x \sin \tau)\bar{\eta}\right) d\eta d\tau \leq \kappa \epsilon,
\end{equation}
we obtain
\begin{equation}
\left| (\sin \tau)^{-l} \left( \frac{\eta}{\varepsilon} \right)^n  \frac{\partial^{s+m} \theta^{0}}{\partial \eta^s \partial \tau^m} \right|_{L_p(\Omega^*)} \leq \kappa \sup_{\tau} |a_{0,-s+m+l+n+1}(\tau)| \varepsilon^{\frac{1}{p}-s}.
\end{equation}

\end{proof}


\begin{comment}
\textbf{Lemma 2.2.} We assume that the following conditions hold:
\[
\frac{\partial^{p1+p2} f}{\partial x^{p1}\partial y^{p2}} = 0 \text{ at } (\pm a,0) \text{ for } 0 \leq 2p1 + p2 \leq -2 +  q, \, p1,p2 \geq 0, \, i,q \geq 0,
\]
where no conditions on \( f \) are needed, if \(  q \leq 1 \). Then the functions
\[
\frac{1}{(\sin \xi)^{q-r}} \frac{d^r v^0}{d\xi^r}
\]
are bounded for \( \xi \in [\pi, 2\pi] \), \( r = 0, \ldots, q \), and thus \( a_{0,q}(\xi) \), defined in (3.13), is bounded. Here \( v^0(\xi) = -u^0(a\cosh R\cos \xi, a\sinh R\sin \xi) \).

\begin{proof} We first consider the case where \( q \geq 2 \). Inserting (2.13a) in (3.17) we can write that
\[
\frac{1}{(\sin \eta)^{q-r}} \frac{d^r v^i}{d\eta^r} = \sum_{\substack{l+s \leq r, \\ l,s \geq 0}} \tilde{g}_{l}^{i}(a\cosh R\cos \xi, a\sinh R\sin \xi) \frac{\partial^{l+s'} f}{\partial x^{l'}\partial y^{s'}}(a\cosh R\cos \xi,  a\sinh R\sin \xi)
\]
for \( l'+s' \leq 2i-1 \), \( l',s' \geq 0 \).

\end{proof}
\end{comment}












In the following lemma and theorem, we illustrate how the compatibility conditions are applied to derive the regularity and boundedness of the solutions. For simplicity, we introduce $v^0$ as follows:
\begin{equation}
v^{0}(\tau)=u^0(a \cosh R \cos \tau, a \sinh R \sin \tau) = \int_{-a \sinh R \sin \tau}^{a \sinh R \sin \tau} f(a \cosh R \cos \tau, s) \, ds, \quad \pi < \tau < 2\pi.
\end{equation}



%\begin{lemma}
\noindent \textbf{Lemma 2.3.}If \( q \leq 1 \) or if the compatibility conditions (\ref{general compatibility condition}) hold for \( 2 + 3n \geq -2 + q \geq 0 \), then \( a_{0,q}(\tau) \) is bounded for \( \tau \in [\pi, 2\pi] \).
%\end{lemma}



\begin{proof}



We aim to establish the general case for any non-negative integer $r$ through induction. Specifically, we derive the following recursive relation of the derivatives of $v^0(\tau)$. 
\begin{comment}
The detailed steps of each induction stage, are in the appendix.
\end{comment}

%\begin{comment}
By using an Inductive approach, we easily obtain
\begin{equation}\label{recursive form}
\frac{d^r v^0 (\tau)}{d \tau^r} = \sum_{\substack{l+s \leq r \\ l, s \geq 0}} c_{ls} (\sin \tau)^{2l-r+s} \frac{\partial^{l+s} u^0}{\partial x^l \partial y^s} (a\cosh R\cos \tau, a\sinh R\sin \tau) + \sum_{0 \leq r' \leq r-1} c_{r'} (\sin \tau)^{r'-r} \frac{d^{r'} v^0 (\tau)}{d \tau^{r'}}.
\end{equation}


To bound the second term on the right-hand side of (\ref{recursive form}), notice that


\begin{equation}
\frac{\partial^l u^0}{\partial x^l}  (x, y) = \sum_{l'+s' \leq l-1, l',s' \geq 0} g_{l'ls'} (x) \frac{\partial^{l'+s'} f}{\partial x^{l'} \partial y^{s'}} (x, C_u(x)) \\
+ c_{l}   \int^{C_u(x)}_{y} \frac{\partial^l f}{\partial x^l}   (x, s) ds,
\end{equation}





\begin{equation}
\left\{ \frac{\partial^s}{\partial y^s} \left[ \frac{\partial^l u^0}{\partial x^l} \right] \right\} (x, y) = \sum_{l'+s' \leq l-1, l',s' \geq 0} g_{l'ls's} (x) \frac{\partial^{l'+s'} f}{\partial x^{l'} \partial y^{s'}} (x, C_u(x)) \\
+ c_{ls} \left\{ \frac{\partial^{s-1}}{\partial y^{s-1}} \left[ \frac{\partial^l f}{\partial x^l} \right] \right\} (x, y),
\end{equation}





where
\begin{align}
\frac{\partial^{-1} f}{\partial y^{-1}}(x,y) &= \int_{y}^{C_u(x)} f(x, s) \, ds, \quad \text{and} \quad \left| g_{l'ls's}(x) \right| \leq \kappa C_u(x)^{-(-1+2l-2l'-s')}.
\end{align}






Then, we rewrite (\ref{recursive form})



\begin{align}\label{recursive form expansion}
\frac{1}{(\sin \tau)^{q-r}} \frac{d^{r} v^0}{d \tau^{r}} (\tau) &= \sum_{\substack{l+s \leq r, l, s \geq 0 \\ l'+s' \leq l-1, l', s' \geq 0}} \tilde{g}_{l'ls's}(a\cosh R\cos \tau) \left( \frac{\partial^{l'+s'}}{\partial x^{l'} \partial y^{s'}} f \right)(a\cosh R\cos \tau, a\sinh R\sin \tau) \nonumber \\
&\quad + \sum_{\substack{l+s \leq r,\\ l, s \geq 0 }} \tilde{c}_{ls} (\sin \tau) \left( \frac{\partial^{s-1}}{\partial y^{s-1}} \left[ \frac{\partial^{l}}{\partial x^{l}} f \right] \right) (a\cosh R\cos \tau, a\sinh R\sin \tau) \nonumber \\
&\quad + \sum_{0 \leq r' \leq r-1} \frac{c_{r'}}{(\sin \tau)^{q-r'}} \frac{d^{r'} v^0(\tau)}{d \tau^{r'}},
\end{align}














\[
\text{where } \left| \tilde{g}_{l'ls's}(a\cosh R\cos \tau) \right| \leq \kappa (\sin \tau)^{-(1-2l'-s'+q-s)} \text{ and } \left| \tilde{c}_{ls}(\sin \tau) \right| \leq \kappa (\sin \tau)^{-(q-2l-s)}.
\]


\noindent Then, since
\[
0 \leq 2(p' + l') + q' + s' \leq -1 + q - s - 1 \leq -2  + q,
\]
it follows that
\begin{equation}
\frac{\partial^{p'+q'}}{\partial x^{p'} \partial y^{q'}} \left( \frac{\partial^{l'+s'}}{\partial x^{l'} \partial y^{s'}} f \right) = 0 \quad \text{at } (\pm a, 0) \quad \text{for } 0 \leq 2p' + q' \leq -1  - 2l' - s' + q - s - 1.
\end{equation}

\noindent Similarly, considering
\[
0 \leq 2(p' + l') + q' + s' - 1 \leq -2 + q,
\]
we deduce that
\begin{equation}
\frac{\partial^{p'+q'}}{\partial x^{p'} \partial y^{q'}} \left( \frac{\partial^{s-1}}{\partial y^{s-1}} \left[ \frac{\partial^{l}}{\partial x^{l}} f \right] \right) = 0 \quad \text{at } (\pm a, 0) \quad \text{for } 2p' + q' \leq q - 2l - s - 1.
\end{equation}
This results in the boundedness of the first and second terms, by using Lemma 2.1.
We demonstrate the boundedness of the third sum on the right-hand side of equation (\ref{recursive form expansion}) using an inductive approach on the variable \( r \).
Consider the sum defined by
\[
S_r = \sum_{0 \leq r' \leq r-1} \frac{c_{r'}}{(\sin \tau)^{q-r'}} \frac{d^{r'} v^0(\tau)}{d \tau^{r'}},
\]
where \( c_{r'} \) are coefficients, \( \tau \) is the variable, and \( v^0 \) is a function of \( \tau \). We aim to show that \( S_r \) is bounded for all \( r \geq 0 \). We proceed by induction on \( r \).

\textbf{Initial Step:} For \( r = 0 \),
\[
S_0 = 0,
\]
as there are no terms in the sum, hence \( S_0 \) is trivially bounded.

\textbf{Inductive Step:} Assume \( S_r \) is bounded for  \( r \geq 0 \).




Consider the sum defined by
\begin{equation}\label{Inductive step}
S_{r+1} = \sum_{0 \leq r' \leq r-1} \frac{c_{r'}}{(\sin \tau)^{q-r'}} \frac{d^{r'} v^0(\tau)}{d \tau^{r'}} + \frac{c_{r-1}}{(\sin \tau)^{q-r+1}} \frac{d^{r-1} v^0(\tau)}{d \tau^{r-1}}.
\end{equation}

If we substitute the right-hand side of (\ref{Inductive step}) with expression (\ref{recursive form expansion}) for \(S_r\), then under the assumption that \(S_r\) is bounded, \(S_{r+1}\) will also be bounded. 
\end{proof}























%\end{equation}
%\end{comment}




















The following property of the derivatives of \( \theta^0 \) is derived from compatibility conditions and Lemma 2.1.
\noindent \textbf{Lemma 2.4.} If \( q \leq 1 \) or if the compatibility conditions (\ref{general compatibility condition}) are satisfied for \( 2 + 3n \geq -2 + q \geq 0 \), then the following inequality is established:




\begin{equation}
\left |(\cosh R-\cosh (R-\eta)) \frac{\partial \theta^0}{\partial \eta} \right|_{L^2(D^*)} \leq \kappa \varepsilon^{\frac{1}{2}}, \notag
\end{equation}
\begin{equation}
\left| \frac{\partial \theta^0}{\partial \tau} \right|_{L^2(D^*)} \leq \kappa \varepsilon^{\frac{1}{2}}. \notag
\end{equation}





\begin{comment}
Assuming (2.1) with \( m = 0 \), from Lemmas 3.2 and 3.5 below with \( j = 0 \), \( \sigma = \varepsilon^{\frac{2}{3}} \), we find that
\end{comment}

\begin{equation}
\left| L_\varepsilon (\theta^0 - \bar{\theta^0}) \right|_{L^2(D^*)} \leq \kappa \varepsilon^{\frac{1}{2}}.
\end{equation}



\begin{comment}
\[
\left| \theta^0 - \bar{\theta^0} \right|_{L^2(D^*)} \leq \kappa \varepsilon,
\]
\[
\left| \frac{\partial}{\partial r} (\theta^0 - \bar{\theta^0}) \right|_{L^2(D^*)} \leq \kappa \varepsilon^{\frac{2}{3}}, \quad \left| \frac{\partial}{\partial \xi} (\theta^0 - \bar{\theta^0}) \right|_{L^2(D^*)} \leq \kappa \varepsilon^{\frac{1}{3}}.
\tag{4.6}
\] 
\end{comment}






\begin{proof}

Applying Lemma 2.1 with \(s=1\), \(m=0\), \(l=0\), and \(n=0\), and using Lemma 2.2 we obtain an upper bound:
\[
\left| \frac{\partial \theta^0}{\partial \eta} \right|_{L^2(D^*)} \leq \kappa \epsilon^{1/2}.
\]
By using the Taylor expansion for \(\cosh R - \cosh (R-\eta)\), we obtain:



\begin{equation}
\left|\left(\cosh R - \cosh (R-\eta)\right) \frac{\partial \theta^0}{\partial \eta} \right|_{L^2(D^*)} \leq \left|\sum_{n=1}^{\infty} \frac{(\epsilon \eta)^n}{n!} \cosh R \right|_{L^2(D^*)} \left|\frac{\partial \theta^0}{\partial \eta}\right|_{L^2(D^*)}.
\end{equation}

Given that \(R < 1\), the series can be bounded by:
\begin{equation}
\left|\left(\cosh R - \cosh (R-\eta)\right) \frac{\partial \theta^0}{\partial \eta} \right|_{L^2(D^*)} \leq  \kappa \left(\sum_{n=1}^{\infty} \epsilon^n\right) \left|\frac{\partial \theta^0}{\partial \eta}\right|_{L^2(D^*)} \leq \kappa \varepsilon^{\frac{1}{2}}.
\end{equation}


Similarly, the boundedness of the derivative with respect to \(\tau\):
\[
\left| \frac{\partial \theta^0}{\partial \tau} \right|_{L^2(D^*)} \leq \kappa \epsilon^{1/2}.
\]
is also easily derived from Lemma 2.1. We now estimate \( L_{\epsilon}(\theta^{0} - \theta^{0}) \). From from Lemmas 2.2, we note that
\begin{align}
\left|\frac{\partial^2 (\theta^{0} - \bar{\theta^{0})}}{\partial \tau^2}\right|_{L^2(D^*_{R/2})} &= \left|\frac{\partial^2 \theta^{0}}{\partial \tau^2} (\delta - R)\right|_{L^2(D^*_{R/2})} \leq \kappa \epsilon^{\frac{1}{2}}, \notag\\
\left|\frac{\partial (\theta^{0} - \bar{\theta^{0})})}{\partial \eta}\right|_{L^2(D^*_{R/2})} &= \left|\frac{\partial \theta^{0}}{\partial \eta} (\delta - R)\right|_{L^2(D^*_{R/2})} + \left|\theta^{0}\frac{\partial (\delta - R)}{\partial \eta}\right|_{L^2(D^*_{R/2})} \leq \kappa \epsilon^{-\frac{1}{2}} + \kappa \epsilon^{\frac{1}{2}} \leq \kappa \epsilon^{-\frac{1}{2}}, \notag\\
\left|\frac{\partial (\theta^{0} - \bar{\theta^{0})})}{\partial \tau}\right|_{L^2(D^*_{R/2})} &= \left|\frac{\partial \theta^{0}}{\partial \tau} (\delta - R)\right|_{L^2(D^*_{R/2})} \leq \kappa \epsilon^{\frac{1}{2}}. 
\end{align}
Using (2.6) and (2.8), we find that
\begin{align}
\left|L_{\epsilon}(\bar{\theta}^{0} - \theta^{0})\right|_{L^2(D^*_{R/2})} \leq {} & \left|\frac{\epsilon}{H} \frac{\partial^2 (\bar{\theta}^{0}  - \theta^{0})}{\partial \tau^2}\right|_{L^2(D^*_{R/2})} \nonumber \\
&+ \left|\frac{a\sinh (R-\eta) \cos \tau}{H} \frac{\partial (\bar{\theta}^{0}  - \theta^{0})}{\partial \tau}\right|_{L^2(D^*_{R/2})} \nonumber \\
&+ \left|\frac{a (\cosh (R-\eta)-\cosh R) \sin \tau}{H} \frac{\partial (\bar{\theta}^{0}  - \theta^{0})}{\partial \eta}\right|_{L^2(D^*_{R/2})} \\
\leq & \kappa \epsilon^{\frac{3}{2}} + \kappa \epsilon^{\frac{1}{2}} + \kappa \epsilon^{\frac{1}{2}} \leq \kappa \epsilon^{\frac{1}{2}}. 
\end{align}
\end{proof}






\noindent \textbf{Theorem 2.5.} The following estimate holds:
\begin{equation}
\left|u^\varepsilon - u^0 - \bar{\theta}^0\right|_{H^1(\Omega)} \leq \kappa \varepsilon^{\frac{1}{2}},
\end{equation}
where \(u^\varepsilon\), \(u^0\) is the solution of (\ref{original pde}), (\ref{limit solution}), and \(\bar{\theta}^0\) is the corrector in (\ref{delta corrector}).



\begin{proof}For the error analysis of solution, writing \( w = u^\varepsilon - u^0 - \bar{\theta}^0 \) from (\ref{Transforemd pde}), (\ref{Approximated corrector equation}) and (\ref{delta corrector}) we deduce that
\begin{equation}
\begin{cases}
  -\varepsilon \Delta w - w_{y} = \text{R.H.S.},\\
  w = 0 \quad \text{on} \quad \partial D.
\end{cases}
\end{equation}



{\color{blue}
Using the approximate form \(\bar{\theta^0} \) for \(\theta^0  \) we write \( L_\varepsilon \bar{\theta^0} = L_\varepsilon \theta^0 + L_\varepsilon ( \bar{\theta^0}-\theta^0) \), and then \( (L_\varepsilon \theta^0, \varphi) = (L_\varepsilon \theta^0, \varphi \delta(\eta)) \) for all \( \varphi \in H^1_0(D) \) where \( (, ) \) is the scalar product in the space \( L^2(D) \) and \( \delta(\eta) \) is a smooth function such that \( \delta(r) = 1 \) if \( \tau \leq R/2 \) and \( \delta(\eta) = 0 \) if \( \tau \geq 3R/4 \). Note that \( \theta^0 = 0 \) for \( \tau \geq R/2 \).
}
We first observe that



\begin{equation}\label{R.H.S}
R.H.S. = \varepsilon \Delta u^0 - L_\varepsilon (\theta^0) + L_\varepsilon (\theta^0 - \bar{\theta^0}).
\end{equation}




Taking the scalar product of (\ref{R.H.S}) with \( e^y w \) we find with \( D^* \):



\begin{align}
\ \varepsilon | w |^2_{H^1(D)} + | w |^2_{L^2(D)} \ &\leq \varepsilon| ( \Delta u^\varepsilon, e^y w \delta(\eta)) | + | (L_\varepsilon (\theta^0), e^y w \delta(\eta)) | + | (L_\varepsilon (\theta^0 - \bar{\theta^0}), e^y w \delta(\eta)) |  \\
&\leq \kappa \varepsilon | u^0 |_{H^1(D)} | w |_{H^1(D)} \notag\\
&+ \left| \left( \frac{1}{H} \left( -\varepsilon \theta_{\tau \tau} - a \sin \tau (\cosh R - \cosh (R-\eta)) \theta_\eta - a \sinh \eta \cos \tau \theta_{\tau} \right), e^y w \delta(\eta) \right) \right|
\notag\\
&+ \left| (L_\varepsilon (\theta^0 - \bar{\theta^0}), e^y w \delta(\eta)) \right| \\
&\leq \kappa \varepsilon | u^0 |_{H^1(D)} | w |_{H^1(D)} 
+ \kappa \varepsilon \left| \frac{\partial \theta^0}{\partial \tau} \right|_{L^2(D^*)} \left( \left| \frac{\partial w}{\partial \tau} \delta(\eta) \right|_{L^2(D^*)} + \left| w \delta(\eta) \right|_{L^2(D^*)}\right) \notag\\
&+ \kappa \left|(\cosh R-\cosh (R-\eta)) \frac{\partial \theta^0}{\partial \eta} \right|_{L^2(D^*)} \left| w \delta(\eta) \right|_{L^2(D^*)} \notag\\
&+ \kappa|\cos \tau \frac{\partial \theta^0}{\partial \tau}|_{L^2(D^*)} \left| w \delta(\eta) \right|_{L^2(D^*)} \notag\\
&+ \kappa\left| L_\varepsilon (\theta^0 - \bar{\theta^0}) \right|_{L^2(D^*_{R/2})} \left| w \delta(\eta) \right|_{L^2(D^*)}.
\end{align}




\begin{comment}
\[
+ \kappa \left( \varepsilon | \nabla_{\xi,r} (\theta^0 - \theta^0) |_{L^2(D^*)} + | \theta^0 - \theta^0 |_{L^2(D^*)} |\nabla_{\xi,r} (w \delta(\xi)) |_{L^2(D^*)} \right).
\]    
\end{comment}


Hence, since \(\left| \frac{\partial w}{\partial \tau} \delta(\eta) \right|_{L^2(D^*)}, \left| \nabla_{\tau, \eta} (w \delta(\eta)) \right|_{L^2(D^*)} \leq \kappa |w|_{H^1(D)}\) and \(\left|w \delta(\eta)\right|_{L^2(D^*)} \leq \kappa |w|_{L^2(D)}\) and using Lemma 2.2.,
we obtain 


\begin{equation}
|w|_{L^2(D)} + \sqrt{\varepsilon} |w|_{H^1(D)} \leq \kappa \sqrt{\varepsilon}.
\end{equation}



\end{proof}
}

==> Convection_diffusion_in_square.tex <==
\section{Convection-Diffusion Equations in a Channel Domain
}




To begin, we examine two-dimensional convection-diffusion equations {in} square domains. To emphasize the presence of the boundary layer, we employ periodic boundary conditions in the $x$ direction and zero boundary conditions in the $y$ direction:
\begin{equation} \label{e:square}
\begin{split}
   - \epsilon \Delta u^{\ep} - u^{\ep}_y & = f, \quad \text{  in  } \Omega=(0,1)\times(0,1), \\
     u^{\ep}  & = 0, \quad \text{  at  } y=0 \text{ and } y=1,\\
     u^{\ep} & \text{ is periodic in }  x.
\end{split}    
\end{equation}
We construct an SL-PINN for the singular perturbation problem and compare its performance with conventional PINNs. To obtain the corrector function, we initiate the process by examining the limit problem, where we set $\epsilon$ to 0 in the governing equation:
\begin{equation} \label{e:square_limit}
\begin{split}
-u^{0}_y & = f \quad \text{  in  } \Omega,\\
u^{0} & =0 \text{ at } y=1,\\
u^{0} & \text{ is periodic in }  x.
\end{split}
\end{equation}
%%%%%%%%%%%%%%%%%%%%
% Put how to derive the corrector equation.
%%%%%%%%%%%%%%%%%%%%
Along the asymptotic analysis, the boundary layers are defined by the inner expansion 
$
u^{\ep} \sim \sum^{\infty}_{j=0} \ep^{j} \theta^{j}.
$
Let $\bar{y} = y / \epsilon$ be considered as an $\mathcal{O}(1)$ quantity in the boundary layer.
\be
    - \sum^{\infty}_{j=0}
    \{
        \ep^{j+1}
        \theta^j_{xx}
        +
        \ep^{j-1}
        \theta^j_{\bar{y} \bar{y}}
    \}
    - \sum^{\infty}_{j=0}
    \ep^{j-1}
        \theta^j_{\bar{y}}
        = 0. 
\ee
By formally identifying each power of $\epsilon$, we can derive the corrector equation by selecting the dominant terms,
\begin{equation} \label{e:square_cor}
\begin{split}
-\ep \varphi^{0}_{{yy}}-\varphi^{0}_{{y}} & =0 \quad \text{  in  } \Omega,\\
\varphi^{0} & =-u^{0}(x,0) \text{ at } y=0, \\
\varphi^{0} & \text{ is periodic in }  x.
\end{split}
\end{equation}
One can easily find an explicit solution of \eqref{e:square_cor} 
\be \label{eq:sq_cor_sol}
    { {\varphi}^0}
    = -u^0(x,0) \frac{e^{-y/\ep} - e^{-1/\ep}}{1 - e^{-1/\ep}}
    = -u^0(x,0) e^{-y/\ep} + e.s.t., 
\ee
where $e.s.t.$ stands for an exponentially small term.
Here, we omit further boundary layer analysis, such as convergence to the limit problem. For more detailed theoretical results, one can refer to the work by {\cite{bookSP},\cite{jung2005numerical}.



We modify the 2-layer PINN in \eqref{e:PINN} based on boundary layer analysis, incorporating the profile of the corrector described in \eqref{eq:sq_cor_sol}.
Our new {\it SL-PINN} is proposed of the form,
\begin{equation}\label{e:app_sol_enriched_con-def}
    \widetilde{u}(x,y ; \, {\blds \theta}) 
            =x(x-1)((y-1) \hat{u}(x,y , {\blds \theta}) +\hat{u}(x,0, {\blds \theta}) { \bar {\varphi}^0}),
\end{equation}
where the corrector function is given by $\bar{\varphi}^0=e^{-\frac{y}{\epsilon}}.$
The residual loss function is defined by
\begin{equation}
\begin{split}
    Loss=\frac{1}{N}\sum_{i=0}^{N}\| L_{\epsilon}(\widetilde{u}(x_i,y_i ; \, {\blds \theta}) )-f(x_i,y_i) \|_{p} \quad  \text{ where }(x_i,y_i) \in \Omega,
\end{split}    
\end{equation}
where $p = 1, 2$.
Using the fact that the exponentially decaying function ${\bar{\varphi}^0}$ satisfies the corrector equation (\ref{e:square_cor}), we can deduce the residual loss:
\begin{equation}  \label{e:square_loss}
\begin{split}
-\ep \Delta \widetilde{u} - \widetilde{u}_y - f
 & = -2\ep((y - 1)\hat{u}(x,y,{\blds \theta})+\hat{u}(x,0,{\blds \theta}){\bar{\varphi}}^0)-\ep (x^2-x)\hat{u}_{xx}(x,0,{\blds \theta}) {\bar{\varphi}}^0 \\
 &-2\ep((2x-1)(y-1)\hat{u}_{x}(x,y , {\blds \theta})+(x^2-x)\hat{u}_{y}(x,y , {\blds \theta}))\\
 &-2\ep(2x-1)\hat{u}_{x}(x,0,{\blds \theta}) {\bar{\varphi}}^0\\ 
 &-\ep (x^2-x)(y-1)(\hat{u}_{xx}(x,y , {\blds \theta})+\hat{u}_{yy}(x,y , {\blds \theta}))-(x^2 - x)(\hat{u}(x,y,{\blds \theta})\\
 &+(y-1)\hat{u}_{y}(x,y , {\blds \theta}))-f.
 \end{split}
 \end{equation}
Hence, the stiff terms of the residual loss are effectively eliminated. It is worth noting that our SL-PINN provides accurate approximations, as all terms in \eqref{e:square_loss} remain bounded as $\ep$ approaches $0$, regardless of the small parameter $\ep$.
\begin{figure}[htbp]
     \centering
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/square_true_3d.png}
         \caption{True solution}
         %\label{fig:three sin x}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/square_3d.png}
         \caption{SL-PINN using $L^2$ training}
         %\label{fig:y equals x}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/square_3d_l1.png}
         \caption{SL-PINN using $L^1$ training}
         %\label{fig:three sin x}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/square_pinn_pred_3d.png}
         \caption{Conventional PINN}
         %\label{fig:three sin x}
     \end{subfigure}
        \caption{Numerical prediction of \eqref{e:square} with $\ep = 10^{-6}$ and $f=\sin(2 \pi x)$. For our simulations, we select a uniform grid of $50$ discretized points in each of the $x$ and $y$ directions.}\label{fig1}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[scale=0.4]{fig/true_vs_pred_square_at_0.25.png}
\caption{The one-dimensional profile of predicted solutions along the line $x = 0.25$.} \label{fig1-1}
\end{figure}



We compare the performance of the standard five-layer PINN approximation with our new SL-PINN approximation. Figure \ref{fig1} displays the numerical solutions of \eqref{e:square} with $\ep = 10^{-6}$ when $ f= \sin 2 \pi x$.
In the conventional PINN approximation, we make use of an $M$-layer neural network, where $M \geq 2$, to enhance the performance. However, Figure \ref{fig1} demonstrates that the conventional PINN method fails to approximate the solution of the singular perturbation problem.
On the other hand, our new scheme, which utilizes only a 2-layer neural network with a small number of neurons, outperforms the conventional PINN. The numerical results shown in Figure \ref{fig1} and Table \ref{tab:1} provide strong evidence that the SL-PINN significantly outperforms the conventional PINN method, thanks to the corrector function embedded in the scheme. It is worth noting that our SL-PINN, enriched with the corrector, produces stable and accurate approximate solutions, regardless of the small parameter $\ep$.
A closer examination can be made by referring to Figure \ref{fig1-1}. The one-dimensional profile of predicted solutions at $x=0.25$ allows for a clear comparison. It is evident from Figure \ref{fig1-1} that the $L^1$ and $L^2$ training approaches provide accurate approximations. However, the conventional PINN falls short in capturing the sharp transition near the boundary layer.

==> Convection_diffusion_on_circular.tex <==
\section{Convection-Diffusion Equations in a Circular Domain
}
We shift our focus to the convection-diffusion equation within a circular domain. We begin by examining the time-independent problem and subsequently delve into the computation of the time-dependent equations.
\subsection{Time-indepedent problem}
We examine the convection-diffusion equation in a circular domain such that
\begin{equation} \label{e:circle_eq}
\begin{split}
   L_{\epsilon}u^{\ep} {:=}- \epsilon \Delta u^{\ep} - u^{\ep}_y & =f, \quad \text{  in  } \Omega=\{(x,y) | x^{2}+y^{2}< 1\}\\
    u^{\ep}  & = 0, \quad \text{  at  } \partial \Omega.
\end{split}    
\end{equation}
The singularly perturbed problem described in equation \eqref{e:circle_eq} requires careful treatment when conducting a boundary layer analysis due to the presence of a degenerate boundary layer near the characteristic points at $(\pm 1,0)$ \cite{hong2014numerical}.
To develop the boundary layer analysis, we utilize the polar coordinates such that
$x=(1-\eta)\cos \tau, y=(1-\eta) \sin \tau$.
By setting $u^{\ep}(x,y)=v^{\ep}(\eta,\tau)$, we derive that
\be
\begin{split}
P_{\epsilon} v^{\epsilon} 
    := \frac{1}{(1-\eta)^2}
    \left(
    -\epsilon \left( v^{\epsilon}_{\tau \tau} - (1-\eta) v^{\epsilon}_{\eta} + (1-\eta)^{2} v^{\epsilon}_{\eta \eta} \right) 
    + (1-\eta)^{2} \sin \tau v^{\epsilon}_{\eta} - (1-\eta) \cos \tau v^{\epsilon}_{\tau}
    \right) = f, \quad  &\text{in } D, \\
v^{\epsilon}(0, \tau) = 0, \quad \text{at } 0 \leq \tau \leq &2\pi,
\end{split}
\ee

where $D:=\{(\eta,\tau)| 0< \eta <1 , 0\leq \tau \leq 2\pi\}$.
For the sake of simplicity, we define the upper semi-circle as
$\Gamma_{+}:= \{ (x, y)|x^2 + y^2 = 1, y > 0\}$ and the lower semi-circle as $\Gamma_{-}:=\{ (x, y)|x^2 + y^2 = 1, y < 0\}$.
Performing the boundary layer analysis as in \cite{hong2014numerical}, we are led to the following equation for the corrector equation
\be \label{e:cor:circle}
\begin{split}
    - \ep \varphi^0_{\eta \eta } + (\sin \tau) \varphi^0_{\eta}  & = 0, \quad \text{  for  } 0 < \eta < 1, \quad 0 < \tau \leq 2 \pi, \\
     \varphi^0  & = - v^0(\cos \tau, \sin \tau), \quad \text{  on  } \Gamma_{-}, \\
     \varphi^0  & \rightarrow 0 \quad \text{ as } \tau \rightarrow 1.
\end{split}
\ee
Hence, we are able to find an explicit solution of the correction equation \eqref{e:cor:circle}:
\be
\varphi^0 = -v^0(\cos\tau \sin\tau)\exp\left(\frac{\sin \tau}{\ep} \eta \right) \chi_{\pi, 2\pi}(\tau),
\ee
where $\chi$ stands for the characteristic function.
To match the boundary condition in our numerical scheme, we introduce a cut-off function to derive an approximate form 
\be
\bar \varphi^0 = \exp\left(\frac{\sin \tau}{\ep} \eta \right) \chi_{\pi, 2\pi}(\tau) \delta(\eta),
\ee
where $\delta(\eta)$ is a smooth cut-off function such that $\delta(\eta) = 1$ for $\eta \in [0, 1/2]$ and $=0$ for $r \in [3/4, 1]$.
We now establish the semi-analytic SL-PINN method as
\begin{equation}\label{e:EPINN_scheme_circle01}
    \widetilde{v}(\eta,\tau ; \, {\blds \theta}) 
            =(\hat{v}(\eta,\tau, {\blds \theta})-\hat{v}(0,\tau, {\blds \theta}) {\bar \varphi^0})C(\eta,\tau),
\end{equation}
where $C(\eta,\tau)$ is given by
\begin{equation} \label{e:circle_C_term}
\begin{split}
    C(\eta,\tau)=\begin{cases}
    1-(1-\eta)^3 , \text{ if } 0 \leq \tau \leq \pi,\\
    1-(1-\eta)^3-((1-\eta)\sin\tau)^3, \text{ if } \pi < \tau <2\pi,
    \end{cases}
\end{split}
\end{equation}
and $\hat{v}(\eta,\tau) = \hat{u}(x,y)$.
Then, the residual loss is defined by
\begin{equation} \label{e:circle_loss_first}
\begin{split}
    Loss=\frac{1}{N}\sum_{i=0}^{N} \| P_{\epsilon}\widetilde{v}((\eta_{i},\tau_{i}; {\blds \theta}))-f \|_{p} \quad  \text{ for }(\eta_{i},\tau_{i}) \in  D,
\end{split}    
\end{equation}
where $p=1,2$.
Since the boundary layer behavior occurs near the lower semi-circle, we divide the residual loss \eqref{e:circle_loss_first} into two parts: $0 \leq \tau \leq \pi$ and $\pi \leq \tau \leq 2 \pi$.
For the case of $0 \leq \tau \leq \pi$, the calculation of the residual loss is straightforward:

\begin{equation} \label{e:DD1c}
\begin{split}
    & P_{\epsilon}\widetilde{v}((\eta,\tau, {\blds \theta})) - f \\
    & =
    -\ep \left(\frac{1}{(1-\eta)^2} - (1-\eta)\right) \hat{v}_{\tau \tau}(\eta, \tau, {\blds \theta}) 
    + \left((1-\eta)^2 - \frac{1}{(1-\eta)}\right) \cos(\tau) \hat{v}_{\tau}(\eta, \tau, {\blds \theta}) \\
    & \qquad -\ep (1 - (1-\eta)^3) \hat{v}_{\eta \eta}(\eta, \tau, {\blds \theta}) \\
    & \qquad - \left(6\ep + \ep (1-\eta)^2 - \frac{\ep}{(1-\eta)} - \sin(\tau)(1 - (1-\eta)^3)\right) \hat{v}_{\eta}(\eta, \tau, {\blds \theta}) \\
    & \qquad + \left(3\ep + \frac{6\ep}{(1-\eta)} + 3 (1-\eta)^2 \sin(\tau)\right) \hat{v}(\eta, \tau, {\blds \theta}) - f,
\end{split}
\end{equation}




where $0 < \eta \leq 1 $ and $0 \leq \tau \leq \pi.$
However, in the case of $\pi \leq \tau \leq 2 \pi$, the introduction of the boundary layer element in \eqref{e:EPINN_scheme_circle01} and the inclusion of the regularizing term in \eqref{e:circle_C_term} complicate the residual loss as follows:\begin{equation}
\begin{split}
    & P_{\epsilon}\widetilde{v}(\eta,\tau, {\blds \theta}) - f \\
    & = -\ep \left( \frac{1}{(1-\eta)^2} - (1-\eta) - (1-\eta) \sin^3(\tau) \right) \hat{v}_{\tau \tau}(\eta, \tau, {\blds \theta}) \\
    & \quad + \left( 6 \ep (1-\eta) \sin^2(\tau) \cos(\tau) + \left( (1-\eta)^2 - \frac{1}{(1-\eta)} + (1-\eta)^2 \sin^3(\tau) \right) \cos(\tau) \right) \hat{v}_{\tau}(\eta, \tau, {\blds \theta}) \\
    & \quad -\ep \left( 1 - (1-\eta)^3 - (1-\eta)^3 \sin^3(\tau) \right) \hat{v}_{\eta \eta}(\eta, \tau, {\blds \theta}) \\
    & \quad - \left( 6\ep + \ep (1-\eta)^2 - \frac{\ep}{(1-\eta)} + 7\ep (1-\eta)^2 \sin^3(\tau) + (1-\eta)^3 \sin^3(\tau) - (1 - (1-\eta)^3) \sin(\tau) \right) \hat{v}_{\eta}(\eta, \tau, {\blds \theta}) \\
    & \quad + \left( 3\ep + \frac{6\ep}{(1-\eta)} + 6 \ep (1-\eta) \sin(\tau) + 6 (1-\eta)^2 \sin(\tau) \right) \hat{v}(\eta, \tau, {\blds \theta}) \\
    & \quad - \hat{v}(0, \tau, {\blds \theta}) \Big[ \ep \left( C(\eta, \tau) \delta_{\eta \eta} - \left( (1-\eta) C(\eta, \tau) - 2 C_{\eta}(\eta, \tau) \right) \delta_{\eta} \right. 
     \quad \left.  -\left( (1-\eta) C_{\eta}(\eta, \tau) - C_{\eta \eta}(\eta, \tau) \right) \delta \right) \\
    & \quad - C(\eta, \tau) \sin(\tau) \delta_{\eta} + C_{\eta}(\eta, \tau) \sin(\tau) \delta \Big] \exp\left( \frac{\sin \tau}{\ep} \eta \right) \\
    & \quad + \frac{\delta}{(1-\eta)^2} \Big[ (\ep \hat{v}_{\tau \tau}(0, \tau, {\blds \theta}) + 1+\eta) \cos(\tau) \hat{v}_{\tau}(0, \tau, {\blds \theta}) - \eta \sin(\tau) \hat{v}(0, \tau, {\blds \theta})) C(\eta, \tau) \\
    & \quad + \left( 2\ep \hat{v}_{\tau}(0, \tau, {\blds \theta}) + (1+\eta)) \cos(\tau) \hat{v}(0, \tau, {\blds \theta}) \right) C_{\tau}(\eta, \tau) + \ep \hat{v}(0, \tau, {\blds \theta}) C_{\tau \tau}(\eta, \tau) \Big] \exp\left( \frac{\sin \tau}{\ep} \eta \right) \\
    & \quad + C(\eta, \tau) \hat{v}(0, \tau, {\blds \theta}) \frac{\delta(\eta)}{(1-\eta)^2} \left( \frac{\eta \cos^2(\tau)}{\ep} \right) \exp\left( \frac{\sin \tau}{\ep} \eta \right) - f,
\end{split} \label{eq:circle:complex}
\end{equation}

where $0<\eta\leq 1$ and $\pi < \tau < 2\pi$.







{\color{red}









To make the computation in \eqref{eq:circle:complex} feasible, we extract the largest order term in $\ep$, which includes $O(\ep^{-1})$ such that
\begin{equation}
    \psi(\eta,\tau,{\blds \theta}) := (1-(1-\eta)^3-(((1-\eta)\sin\tau)^3)\hat{v}(0,\tau,{\blds \theta})\frac{\delta(\eta)}{(1-\eta)^2} \left(\frac{\eta}{\ep}\cos^2\tau \right) \exp\left(\frac{\sin \tau}{\ep} \eta \right).
\end{equation}


\begin{remark}
It holds that
\[
    \left\| \frac{1}{\epsilon} \exp\left( \frac{\sin \tau}{\epsilon} \eta \right) \right\|_{L^{1}(D^{*})} < C_{1},
\]
where \(C_{1}, C_{2}\) are constants.
\end{remark}








By the triangular inequality, the loss in \eqref{e:circle_loss_first} becomes 
\begin{equation}\label{e:bound00}
 Loss  \leq \frac{1}{N}\sum_{i=0}^{N}|\psi (\eta_{i},\tau_{i},{\blds \theta})|
 +  \frac{1}{N}\sum_{i=0}^{N} |P_{\epsilon}\widetilde{v}((\eta_{i},\tau_{i},{\blds \theta}))-\psi (\eta_{i},\tau_{i},{\blds \theta})-f|,
\end{equation}
The rightmost term does not include a large order term such as ${\ep^{\alpha}}$ (where $\alpha < 0$) since $\psi$ contains the large terms such as $\ep^{-1}$. Hence, this part can be computed using conventional $L^1$ or $L^2$ loss. Since $\psi$ contains $\mathcal{O}(\epsilon^{-1})$, we handle $\psi$ using $L^1$ loss. More precisely, let us suppose we choose the number of sampling points $N$ to be sufficiently large
\begin{equation}\label{e:bound01}
\begin{split}
     & \frac{1}{N}\sum_{i=0}^{N}|\psi(\eta_{i},\tau_{i},{\blds \theta})| \approx \frac{1}{\pi}\int^{2\pi}_{\pi} \int^{1}_{0} |\psi(\eta,\tau,{\blds \theta})|d \eta d \tau.\\
\end{split}
\end{equation}
The right-hand side of equation (\ref{e:bound01}) is bounded by \(C_1 + C_2 \epsilon\), by using the Remark 4.1.
Particularly, we obtain

\begin{comment}
Note that $\delta(r)$ is a smooth cut-off function such that $\delta(r) = 1$ for $r \in [3/4, 1]$ and $=0$ for $r \in [0, 1/2]$,

By setting $\frac{1-r}{\ep}=\overline{r}$, we have 
\end{comment}
\begin{equation}\label{e:bound03}
\begin{split}
     \frac{1}{\pi}\int^{2\pi}_{\pi} \int^{1}_{0} | \psi(\eta,\tau,{\blds \theta})|d \eta d \tau
     & \leq \frac{K}{2}+K\ep e^{-\frac{1}{2\ep}}-K\ep.
\end{split}
\end{equation}}
Thus, in \eqref{e:bound00}, we focus on minimizing the rightmost term, as the first term on the right-hand side of \eqref{e:bound00} becomes nearly constant by \eqref{e:bound03} when $\ep$ is sufficiently small.
This simplification enables feasible computations in our analysis.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/circle_compatible_true_3d.png}
         \caption{True solution}
         %\label{fig:three sin x}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/circle_compatible_epinn_3d.png}
         \caption{SL-PINN using $L^2$ training}
         %\label{fig:y equals x}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/circle_compatible_epinn_3d_l1.png}
         \caption{SL-PINN using $L^1$ training}
         %\label{fig:three sin x}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/circle_compatible_pinn_3d.png}
         \caption{Conventional PINN}
         %\label{fig:three sin x}
     \end{subfigure}
        \caption{Numerical prediction of \eqref{e:circle_eq} with $\ep = 10^{-6}$ and $f=(1-x^2)^2$. For our simulations, we select a uniform grid of $50$ discretized points in each of the $\eta$ and $\tau$ directions.}\label{fig2}
\end{figure}



The performance of our new approach is demonstrated through a series of numerical experiments in Figure (\ref{fig2})-(\ref{fig4}). For numerical experiments, we choose $50$ uniformly discretized grid points to be used in each $\tau$ and $\eta$ direction.
It is important to note that if $f$ does not vanish at the characteristic points $(\pm 1, 0)$, the function $f(x, y)$ becomes incompatible due to the emergence of singularities in its derivatives at these points.
For the sake of simplicity, in this paper, we consider the first compatibility condition, that is, 
\be
    \frac{\partial^{p_1 + p_2} f}{\partial x^{p_1} \partial y^{p_2}} = 0, \quad \text{at  } (\pm 1, 0), 
\ee
for $0 \leq 2 p_1 + p_2 \leq 2$ and $p_1, p_2 \geq 0$.
For more details on compatibility conditions, see e.g. \cite{hong2014numerical}.
%We first compute the compatible case, i.e., $f = (1-x^2)^2$ in Figure \ref{fig2}.
We compare the performance of the standard five-layer PINN approximation with our SL-PINN approximation. Figure \ref{fig2} displays the numerical solutions of \eqref{e:circle_eq} with $\ep = 10^{-6}$ when $f = (1-x^2)^2$.
Figure \ref{fig2} clearly illustrates the failure of the conventional PINN method in approximating the solution of the singular perturbation problem.
On the contrary, our SL-PINN significantly outperforms the conventional PINN method. 
The numerical results depicted in Figure \ref{fig2} and Table \ref{tab:1} offer compelling evidence that the semi-analytic SL-PINN outperforms the conventional PINN method significantly. 
This improvement is attributed to the incorporation of a corrector function within the scheme. 
Our SL-PINN, enriched with the corrector, consistently generates stable and accurate approximate solutions, irrespective of the small parameter $\ep$. 

\begin{figure}%[htbp]
\centering
\includegraphics[scale=0.4]{fig/true_vs_pred_circle_compatible_at_0.5pi.png}
\caption{The one-dimensional profile of predicted solutions along the line $\tau = \pi/2$.} \label{fig2-2}
\end{figure}

















































For a more detailed analysis, Figure \ref{fig2-2} provides a closer examination of the one-dimensional profile of predicted solutions at $\tau=\pi/2$, enabling a clear and direct comparison.
Figure \ref{fig2-2} clearly demonstrates that both the $L^1$ and $L^2$ training approaches yield highly accurate approximations. However, the conventional PINN method falls short when it comes to capturing the sharp transition near the boundary layer.










To delve deeper into the subject, we consider a non-compatible case where $f=1$, as shown in Figure \ref{fig3}. As mentioned earlier, this non-compatible case introduces an additional singularity when $f$ does not vanish at the characteristic points $(\pm 1, 0)$. Analyzing the boundary layer in this scenario requires careful treatment, as discussed in \cite{JT13}. However, our SL-PINN approach effectively resolves the boundary layer behavior, surpassing the limitations posed by theoretical singularities.
We compare the performance of the standard five-layer PINN approximation with our novel SL-PINN approximation. Figure \ref{fig3} clearly demonstrates the failure of the conventional PINN method in accurately approximating the solution of the singular perturbation problem. In contrast, our SL-PINN, utilizing a 2-layer neural network with a small number of neurons, significantly outperforms the conventional PINN method. The numerical results presented in Figure \ref{fig3} and Table \ref{tab:1} provide compelling evidence of the superior performance of our SL-PINN approach over the conventional PINN method.
For a closer examination, Figure \ref{fig3-3} provides a detailed one-dimensional profile of the predicted solutions at $\tau=\pi/2$, enabling a clear and direct comparison. Moreover, Figure \ref{fig3-3} shows the highly accurate approximations obtained through both the $L^1$ and $L^2$ 
\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/circle_non_compatible_true_3d.png}
         \caption{True solution}
         %\label{fig:three sin x}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/circle_non_compatible_epinn_3d.png}
         \caption{SL-PINN using $L^2$ training}
         %\label{fig:y equals x}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/circle_non_compatible_epinn_3d_l1.png}
         \caption{SL-PINN using $L^1$ training}
         %\label{fig:three sin x}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/circle_non_compatible_pinn_3d.png}
         \caption{Conventional PINN}
         %\label{fig:three sin x}
     \end{subfigure}
        \caption{Numerical prediction of \eqref{e:circle_eq} with $\ep = 10^{-6}$ and $f=1$ (non-compatible case). For our simulations, we select a uniform grid of $50$ discretized points in each of the $\eta$ and $\tau$ directions.}\label{fig3}
\end{figure}

training approaches. However, the conventional PINN method falls short in capturing the sharp transition near the boundary layer.




As an illustrative example, we utilize our SL-PINN method to tackle a complex solution profile:
\be \label{e:f_oscillation}
    u^{\ep}=-A(x)(y+\sqrt{1-x^2})(1-e^{\frac{-2A(x)\sqrt{1-x^2}}{\epsilon}})+2A(x)(\sqrt{1-x^2})(1-e^{\frac{-A(x)(y+\sqrt{1-x^2})}{\epsilon}})
\ee 
In this specific case, the corresponding forcing term can be obtained through direct computation. Due to the presence of multiple humps in the exact solution, the numerical solution displays oscillatory profiles, as depicted in Figure \ref{fig4}. However, our SL-PINN method effectively captures both the solution profile and the sharp transition near the boundary layer. We have excluded the numerical experiments with the conventional PINN approach since it consistently fails to produce an accurate solution profile.


\begin{figure}[H]
\centering
\includegraphics[scale=0.4]{fig/true_vs_pred_circle_non_compatible_at_0.5pi.png}
\caption{The one-dimensional profile of predicted solutions along the line $\tau = \pi/2$.} \label{fig3-3}
\end{figure}

\begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/oscillation_true_3d.png}
        \caption{True solution}
         %\label{fig:y equals x}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/oscillation_epinn_3d.png}
        \caption{SL-PINN using $L^2$ training}
         %\label{fig:three sin x}
    \end{subfigure}
        \caption{Numerical prediction of \eqref{e:circle_eq} with $\ep = 10^{-6}$ and $f$ specified in \eqref{e:f_oscillation}. For our simulations, we select a uniform grid of $50$ discretized points in each of the $\eta$ and $\tau$ directions.}\label{fig4}
\end{figure}











\subsection{Time-depedent problem}
We extend our approach to {a} time dependent problem
\begin{equation} \label{e:time_circle}
\begin{split}
   L_{\epsilon}u^{\ep} :u^{\ep}_{t}- \epsilon \Delta u^{\ep} - u^{\ep}_y & =f, \quad \text{ for } (x,y) \in \Omega, \quad t \in (0,T),\\
     u^{\ep}(x,y,t)  & = 0, \quad \text{  for  } (x,y) \in \partial \Omega, \quad t \in (0,T),\\
     u^{\ep}(x,y,0) & =0, \quad \text{ for } (x,y) \in \Omega, \quad \text{ at } t=0.\\
\end{split}    
\end{equation}
We employ polar coordinates, expressed as $x=(1-\eta)\cos \tau$ and $y=(1-\eta) \sin \tau$, in order to facilitate the development of the boundary layer analysis. By introducing the transformation $u^{\ep}(x,y,t)=v^{\ep}(\eta,\tau,t)$, we obtain that
\begin{comment}
\begin{equation}
\begin{split}
P_{\epsilon}v^{\ep}=v^{\ep}_{t}+\frac{1}{(1-\eta)^2}(-\epsilon(v^{\ep}_{\tau \tau}-(1-\eta) v^{\ep}_{\eta}+(1-\eta)^{2}v^{\ep}_{\eta \eta} )+(1-\eta)^{2}(\sin \tau) v^{\ep}_{\eta}-(1-\eta) (\cos \tau) v^{\ep}_{\tau})& = f\\, \quad  \text{ in }(\eta,\tau) \in D, t\in (0,T),\\
    v^{\ep}(1,\tau,t)=0, \quad  &\text{ at } 0 \leq \tau \leq 2\pi, t\in (0,T),\\
    v^{\ep}(\eta,\tau,0)=0, \quad  &\text{ in }(\eta
    ,\tau) \in D.
\end{split}
\end{equation}
\end{comment}

\begin{equation}
\begin{aligned}
P_{\epsilon}v^{\epsilon} =  \ v^{\epsilon}_{t} + \frac{1}{(1-\eta)^2} ( -\epsilon ( v^{\epsilon}_{\tau \tau} 
- (1-\eta) v^{\epsilon}_{\eta} + (1-\eta)^2 v^{\epsilon}_{\eta \eta} ) + (1-\eta)^2 (\sin \tau) &v^{\epsilon}_{\eta} - (1-\eta) (\cos \tau) v^{\epsilon}_{\tau} ) = f\\, \quad  &\text{in } (\eta, \tau) \in D, \ t \in (0,T), \\
v^{\epsilon}(0, \tau, t) =  \ 0, \quad  &\text{at } 0 \leq \tau \leq 2\pi, \ t \in (0,T), \\
v^{\epsilon}(\eta, \tau, 0) =  \ 0, \quad  &\text{in } (\eta, \tau) \in D.
\end{aligned}
\end{equation}









As stated in the boundary layer analysis conducted by \cite{hong2015singular}, the sharp transition occurs solely in the spatial direction. Consequently, the solution does not exhibit a boundary layer in the temporal direction.
Therefore, the time-independent problem yields the same form of the corrector equation as in the case without time dependence.
Hence, we can derive the corrector equation as described \cite{hong2015singular}: For each $t>0$,
\be
\begin{split}
     - \ep \varphi^0_{\eta \eta} +(\sin \tau) \varphi^0_{\eta}  & = 0, \quad \text{  for  } (\eta,\tau) \in D  \\
     \varphi^0  & = - v^0(\cos \tau, \sin \tau), \quad \text{  for  } (\eta, \tau) \in \Gamma_{-} ,\\
     \varphi^0  & \rightarrow 0 \quad \text{ as } \eta \rightarrow 1.
\end{split}
\ee
Hence, we are able to find an explicit solution to the correction equation:
\be
\varphi^0 = -v^0(t,\cos\tau, \sin\tau)\exp\left(\frac{\sin \tau}{\ep} \eta \right) \chi_{[\pi, 2\pi]}(\tau),
\ee
where $\chi$ stands for the characteristic function.
For our numerical scheme, we introduce an approximate form,
\be
\bar \varphi^0 = \exp\left(\frac{\sin \tau}{\ep} \eta \right) \chi_{\pi, 2\pi}(\tau) \delta(\eta),
\ee
where $\delta(\eta)$ is a smooth cut-off function such that $\delta(\eta) = 1$ for $r \in [0, 1/2]$ and $=0$ for $\eta \in [3/4, 1]$.
We establish the {\it SL-PINN} based on boundary layer analysis, incorporating the profile of the corrector such that
\begin{equation}\label{e:EPINN_scheme_time}
    \widetilde{v}(t, \eta,\tau ; \, {\blds \theta}) 
            =(e^t-1)
            \left(\hat{v}(t, \eta,\tau,{\blds \theta})-\hat{v}(t, 0,\tau,{\blds \theta}){\bar \varphi^0(\eta,\tau)}\right)C(\eta,\tau),
\end{equation}
where $C(\eta,\tau)$ is given by
\begin{equation}\label{e:circle_time_C_term}
\begin{split}
    C(\eta,\tau)=\begin{cases}
    1-(1-\eta)^3 , \text{ if } 0 \leq \tau \leq \pi\\
    1-(1-\eta)^3-((1-\eta)\sin\tau)^3, \text{ if } \pi < \tau <2\pi,
    \end{cases}
\end{split}
\end{equation}
and $\hat{v}(t,\eta,\tau,{\blds \theta}) = \hat{u}(t,x,y,{\blds \theta}) = W_{4}{\sigma}(W_{1}x+W_{2}y+W_{3}t+b)$.
Then, the residual loss is defined by
\begin{equation}\label{e:circle_loss_time}
\begin{split}
    Loss=\frac{1}{N}\sum_{i=0}^{N} \|P_{\epsilon}\widetilde{v}((t_i,\eta_{i},\tau_{i},{\blds \theta}))-f \|_{p} \quad  \text{ for }(t_i,\eta_{i},\tau_{i}) \in  [0,T] \times D,
\end{split}    
\end{equation}
where $p=1,2$.
Due to the boundary layer behavior near the lower semi-circle, we split the residual loss \eqref{e:circle_loss_time} into two sections: $0 \leq \tau \leq \pi$ and $\pi \leq \tau \leq 2 \pi$. For the $0 \leq \tau \leq \pi$, calculating the residual loss is simple:
\begin{equation}
\begin{split}\label{e:EPINN_circle_direct_calculation_upper}
    & P_{\epsilon}\widetilde{v}((t,1-\eta,\tau,{\blds \theta})) - f \\
    & = \left( e^{t} \hat{v} + (e^{t} - 1) \hat{v}_{t}(t,\eta,\tau,{\blds \theta}) \right) (1 - (1-\eta)^3) \\
    & \quad + (e^{t} - 1) \left( -\ep \left( \frac{1}{(1-\eta)^2} - (1-\eta) \right) \hat{v}_{\tau \tau}(t,\eta,\tau,{\blds \theta}) 
    + \left( (1-\eta)^2 - \frac{1}{(1-\eta)} \right) \cos(\tau) \hat{v}_{\tau}(t,\eta,\tau,{\blds \theta}) \right. \\
    & \quad - \ep (1 - (1-\eta)^3) \hat{v}_{\eta \eta}(t,\eta,\tau,{\blds \theta}) 
    - \left( 6\ep + \ep (1-\eta)^2 - \frac{\ep}{(1-\eta)} - \sin(\tau) (1 - (1-\eta)^3) \right) \hat{v}_{\eta}(t,\eta,\tau,{\blds \theta}) \\
    & \quad + \left. \left( 3\ep + \frac{6\ep}{(1-\eta)} + 3 (1-\eta)^2 \sin(\tau) \right) \hat{v}(t,\eta,\tau,{\blds \theta}) \right) - f \\
    & \text{for } 0 < \eta\leq 1 ,\quad 0 \leq \tau \leq \pi, \quad 0 \leq t \leq T,
\end{split}
\end{equation}




where $0 < \eta \leq 1 $ and $0 \leq \tau \leq \pi.$
Introducing the boundary layer element in equation \eqref{e:EPINN_scheme_time} and adding the regularizing term in equation \eqref{e:circle_time_C_term} makes the residual loss calculation more complex when 
$\tau$ ranges from $\pi$ to $2\pi$ such that


\begin{equation}\label{e:EPINN_circle_direct_calculation}
\begin{split}
    & P_{\epsilon}\widetilde{v}(t,\eta,\tau,{\blds \theta}) - f \\
    & = \left( e^{t} \hat{v}(t,\eta,\tau,{\blds \theta}) + (e^{t} - 1) \hat{v}_{t}(t,\eta,\tau,{\blds \theta}) 
    - \left( e^{t} \hat{v}(t,0,\tau,{\blds \theta}) + (e^{t} - 1) \hat{v}_{t}(t,0,\tau,{\blds \theta}) \right) \right) \\
    & \quad \times \exp\left( \frac{\sin \tau}{\ep} \eta \right) (1 - (1-\eta)^3 - (1-\eta)^3 \sin^3(\tau)) \\
    & \quad + (e^{t} - 1) \left( -\ep \left( \frac{1}{(1-\eta)^2} - (1-\eta) - (1-\eta) \sin^3(\tau) \right) \hat{v}_{\tau \tau}(t,\eta,\tau,{\blds \theta}) \right. \\
    & \quad + \left( 6 \ep (1-\eta) \sin^2(\tau) \cos(\tau) + \left( (1-\eta)^2 - \frac{1}{(1-\eta)} + (1-\eta)^2 \sin^3(\tau) \right) \cos(\tau) \right) \hat{v}_{\tau}(t,\eta,\tau,{\blds \theta}) \\
    & \quad -\ep \left( 1 - (1-\eta)^3 - (1-\eta)^3 \sin^3(\tau) \right) \hat{v}_{\eta \eta}(t,\eta,\tau,{\blds \theta}) \\
    & \quad + \left( 6\ep + \ep (1-\eta)^2 - \frac{\ep}{(1-\eta)} + 7\ep (1-\eta)^2 \sin^3(\tau) + (1-\eta)^3 \sin^3(\tau) - (1 - (1-\eta)^3) \sin(\tau) \right) \hat{v}_{\eta}(t,\eta,\tau,{\blds \theta}) \\
    & \quad + \left( 3\ep + \frac{6\ep}{(1-\eta)} + 6 \ep (1-\eta) \sin(\tau) + 6 (1-\eta)^2 \sin(\tau) \right) \hat{v}(t,\eta,\tau,{\blds \theta}) \\
    & \quad + \hat{v}(t,0,\tau,{\blds \theta}) \big[ \ep (C(\eta,\tau) \delta_{\eta \eta} + ((1-\eta) C(\eta,\tau) + 2 C_{\eta}(\eta,\tau)) \delta_{\eta} \\
    & \quad - ((1-\eta) C_{\eta}(\eta,\tau) + C_{\eta \eta}(\eta,\tau)) \delta ) - C(\eta,\tau) \sin(\tau) \delta_{\eta} + C_{\eta}(\eta,\tau) \sin(\tau) \delta \big] \exp\left( \frac{\sin \tau}{\ep} \eta \right) \\
    & \quad + \frac{\delta}{(1-\eta)^2} \big[ (\ep \hat{v}_{\tau \tau}(t,0,\tau,{\blds \theta}) + (2+\eta) \cos(\tau) \hat{v}_{\tau}(t,0,\tau,{\blds \theta}) - \eta \sin(\tau) \hat{v}(t,0,\tau,{\blds \theta})) C(\eta,\tau) \\
    & \quad + (2\ep \hat{v}_{\tau}(t,0,\tau,{\blds \theta}) + (1+\eta) \cos(\tau) \hat{v}(t,0,\tau,{\blds \theta})) C_{\tau}(\eta,\tau) + \ep \hat{v}(t,0,\tau,{\blds \theta}) C_{\tau \tau}(\eta,\tau) \big] \exp\left( \frac{\sin \tau}{\ep} \eta \right) \\
    & \quad + (e^{t} - 1) C(\eta,\tau) \hat{v}(t,0,\tau,{\blds \theta}) \frac{\delta(\eta)}{(1-\eta)^2} \left( \frac{\eta \cos^2(\tau)}{\ep} \right) \exp\left( \frac{\sin \tau}{\ep} \eta \right) - f,
\end{split}
\end{equation}







where $0<\eta\leq 1$, $\pi < \tau < 2\pi$, $0 \leq t \leq T$. 
We make computation feasible in equation \eqref{e:EPINN_circle_direct_calculation} by extracting the largest order term in $\ep$, which includes $O(\ep^{-1})$ such that
{\color{red}
\begin{equation}
    \psi(t,\eta,\tau,{\blds \theta})=(e^{t}-1)(1-(1-\eta)^3-(((1-\eta)\sin\tau)^3)\hat{v}(t,0,\tau,{\blds \theta})\frac{\delta(\eta)}{(1-\eta)^2}(\frac{\eta}{\ep}\cos^2\tau)\exp\left(\frac{\sin \tau}{\ep} \eta \right).
\end{equation}
% We now define the loss as follows for the lower semicircle
% \begin{equation}
% \begin{split}
%     Loss=\frac{1}{N}\sum_{i=0}^{N}|P_{\epsilon}\widetilde{v}((t_{i},r_{i},\xi_{i},{\blds \theta}))-f |, \quad  \text{ for }(r_{i},\xi_{i}) \in  D.
% \end{split}    
% \end{equation}
By the triangular inequality, we deduce that
\begin{equation} \label{e:bound_time_0}
 Loss  \leq \frac{1}{N}\sum_{i=0}^{N}|\psi (t_{i},\eta_{i},\tau_{i},{\blds \theta})|
 +  \frac{1}{N}\sum_{i=0}^{N} |P_{\epsilon}\widetilde{v}((t_{i},\eta_{i},\tau_{i},{\blds \theta}))-\psi (t_{i},\eta_{i},\tau_{i},{\blds \theta})-f|,
\end{equation}
The rightmost term does not include a large order term, ${\ep^{\alpha}}$ where $\alpha < 0$, because $\psi$ already accounts for the large terms such as $\ep^{-1}$. 
Therefore, conventional $L^1$ or $L^2$ loss can be used to compute this part. 
As $\psi$ contains $\mathcal{O}(\epsilon^{-1})$, we employ $L^1$-loss to handle $\psi$. Specifically, we choose a sufficiently large number of sampling points $N$ to derive
\begin{equation}\label{e:bound00 time}
\begin{split}
     & \frac{1}{N}\sum_{i=0}^{N}|\psi(t_{i},\eta_{i},\tau_{i},{\blds \theta})| \approx \frac{1}{T \pi}\int^{T}_{0}\int^{2\pi}_{\pi} \int^{1}_{0} |\psi(t,\eta,\tau,{\blds \theta})|d \eta d \tau d t.\\
\end{split}
\end{equation}
The right-hand side of equation (\ref{e:bound00 time}) is bounded by \(C_1 \), by using the Remark 4.1.

By employing calculations similar to those presented in equations \eqref{e:bound01} to \eqref{e:bound03}, we can deduce the following result:
\begin{equation} \label{e:bound_time_1}
\begin{split}
     \frac{1}{T \pi}\int^{T}_{0}\int^{2\pi}_{\pi} \int^{1}_{0} |\psi(t,\eta,\tau,{\blds \theta})|d \eta d \tau d t
     \leq \frac{K}{2}+K\ep e^{-\frac{1}{2\ep}}-K\ep.
\end{split}
\end{equation}}
Thus, in \eqref{e:bound_time_0}, we focus on minimizing the rightmost term, as the first term on the right-hand side of \eqref{e:bound_time_0} becomes nearly constant by \eqref{e:bound_time_1} when $\ep$ is sufficiently small.
This simplification enables feasible computations in our analysis.


The effectiveness of our new approach is demonstrated through a series of numerical experiments, as shown in Figure \ref{fig5}. 
For these experiments, we employ a grid discretization consisting of $50$ uniformly spaced grid points in each direction of $\tau$, $\eta$, and $t$. 
The function $f$ used in these experiments satisfies the compatibility condition mentioned in \cite{hong2015singular}:
\be \label{e:time_force}
f=(1-x^2)^2 t+(1-x^2)^{2}(-y+\sqrt{1-x^2}+\frac{\epsilon(y+\sqrt{1-x^2})}{(1-x^2)^{3/2}})+O(\epsilon).
\ee
Also, the corresponding $u$ is given by
\begin{equation}
\begin{split}
    u(t,x,y)=\begin{cases}
    t(1-x^{2})^{2}(-y+\sqrt{1-x^2}+\epsilon \frac{(y+\sqrt{1-x^2})}{(1-x^2)^{3/2}} , \text{ in } D\\
    0, \text{ on }\partial D.
    \end{cases}
\end{split}
\end{equation}
Figure \ref{fig5} presents the numerical solution obtained using SL-PINN with $\ep = 10^{-6}$. 
In contrast, the conventional PINNs are not included in the figure due to their significant deviation from the true solution.
The SL-PINN, enhanced with the corrector function, consistently produces stable and accurate approximate solutions, irrespective of the small parameter $\epsilon$. Figure \ref{fig5} (C) depicts the one-dimensional predicted solution profiles at $\tau=\pi/2$ for various time instances, including $t=0.25, 0.5, 0.75$, and $1.0$, alongside the true solution. This example serves as evidence that our SL-PINN method delivers accurate predictions throughout the entire time span.




\begin{figure}%[htbp]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/time_true_3d_at_t_1.0.png}
        \caption{True soltuion at t=1}
         %\label{fig:y equals x}
    \end{subfigure}
     %\hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/time_epinn_3d_at_t_1.0.png}
        \caption{SL-PINN at t=1}
         %\label{fig:three sin x}
    \end{subfigure}
     %\hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/true_vs_pred_time_at_0.5pi.png}
        \caption{1D solution profiles}
         %\label{fig:five over x}
    \end{subfigure}
        \caption{Numerical prediction of \eqref{e:time_circle} with $\ep = 10^{-6}$ and $f$ specified in \eqref{e:time_force}. For our simulations, we select a uniform grid of $50$ discretized points in each of the $r$ and $\tau$ directions. In the panel (c), the one-dimensional predicted solution profiles are displayed at $\tau = \pi/2$ for various time instances, including $t = 0.25, 0.5, 0.75$, and $1.0$.}\label{fig5}
\end{figure}















{\color{red}


\subsection{Non-linear problem}
We focus on the non-linear convection-diffusion equation in a circular domain:
\begin{equation}
    - \epsilon \Delta u^{\ep} - u^{\ep}_y+(u^{\ep})^{3} = f \text{ in } \Omega=\{(x,y) | x^{2}+y^{2}< 1\}, \quad u^{\ep} = 0 \text{ on } \partial \Omega.
\end{equation}

Employing polar coordinates \(x=(1-\eta)\cos \tau, y=(1-\eta) \sin \tau\), and substituting \(u^{\ep}(x,y)=v^{\ep}(\eta,\tau)\), the transformed equation is:


\begin{equation}
\begin{split}
P_{\epsilon} v^{\epsilon} 
    := \ \frac{1}{(1-\eta)^2} (
    -\epsilon ( v^{\epsilon}_{\tau \tau} - (1-\eta) v^{\epsilon}_{\eta} + (1-\eta)^{2} v^{\epsilon}_{\eta \eta} ) + (1-\eta)^{2} \sin \tau v^{\epsilon}_{\eta} - (1-\eta) \cos \tau v^{\epsilon}_{\tau} &+  (1-\eta)^{2} (v^{\epsilon})^3
    ) \\
    & = f, \quad \text{in } D, \\
v^{\epsilon}(0, \tau)  = 0, \quad &\text{at } 0 \leq \tau \leq 2\pi,
\end{split}
\end{equation}



The corrector equation in the boundary layer analysis, unaffected by the non-linear term, is:
\begin{equation}
     \ep \varphi^0_{\eta \eta} - (\sin \tau) \varphi^0_{\eta} = 0, \quad \varphi^0 = - v^0 \text{ on } \Gamma_{-}, \quad \varphi^0 \to 0 \text{ as } \eta \to 1,
\end{equation}
with the explicit solution:
\begin{equation}
    \varphi^0 = -v^0\exp\left(\frac{\sin \tau}{\ep} \eta \right) \chi_{[\pi, 2\pi]}(\tau).
\end{equation}

The semi-analytic SL-PINN method is defined as:
\begin{equation}
    \widetilde{v}(\eta,\tau ; \, {\blds \theta}) = (\hat{v}-\hat{v}(0,\tau) {\bar \varphi^0})C(\eta,\tau),
\end{equation}
with the residual loss given by:
\begin{equation}
    Loss=\frac{1}{N}\sum_{i=0}^{N} \| P_{\epsilon}\widetilde{v}(\eta_{i},\tau_{i}; {\blds \theta})-f \|_{p}.
\end{equation}
Here, \( C(\eta,\tau) \) is a function same as \ref{e:circle_C_term}.
The residual loss was calculated in similar fashion.


Figure \ref{fig non-li} presents the numerical solution obtained using SL-PINN with $\ep = 10^{-6}$. 
Unlike conventional PINNs, which struggle to capture the boundary layer, the SL-PINN, enhanced with the corrector function, consistently produces stable and accurate approximate solutions, irrespective of the small $\epsilon$.


\begin{comment}
\begin{equation} \label{e:DD1c}
\begin{split}
    & P_{\epsilon}\widetilde{v}((r,\xi, {\blds \theta})) - f \\
    & =
    -\ep (\frac{1}{r^2}-r)\hat{v}_{\xi \xi}(r,\xi, {\blds \theta})+(r^2-\frac{1}{r}     )\cos(\xi)\hat{v}_{\xi}(r,\xi, {\blds \theta})-\ep(1-r^3)\hat{v}_{r r}(r,\xi, {\blds \theta}) \\
    & \qquad +(6\ep+\ep r^2-\frac{\ep}{r}-\sin(\xi)(1-r^3)      )\hat{v}_{r}(r,\xi, {\blds \theta})
    +(3\ep+\frac{6\ep}{r}+3 r^2 \sin(\xi)  )\hat{v}(r,\xi, {\blds \theta})-f,
\end{split}
\end{equation}
\end{comment}



}

==> Convection_diffusion_on_circular_non_linear.tex <==
\section{Convection-diffusion equations on a circular non linear}
{\color{red}
\subsection{Non-linear problem}
We examine the convection-diffusion equation in a circular domain such that
\begin{equation} \label{e:circle_eq}
\begin{split}
   L_{\epsilon}u^{\ep} {:=}- \epsilon \Delta u^{\ep} - u^{\ep}_y+(u^{\ep})^{3} & =f, \quad \text{  in  } \Omega=\{(x,y) | x^{2}+y^{2}< 1\}\\
    u^{\ep}  & = 0, \quad \text{  at  } \partial \Omega.
\end{split}    
\end{equation}
The singularly perturbed problem described in equation \eqref{e:circle_eq} requires careful treatment when conducting a boundary layer analysis due to the presence of a degenerate boundary layer near the characteristic points at $(\pm 1,0)$ \cite{hong2014numerical}.
To develop the boundary layer analysis, we utilize the polar coordinates such that
$x=r\cos \xi, y=r \sin \xi$.




By setting $u^{\ep}(x,y)=v^{\ep}(r,\xi)$, we derive that
\begin{equation}
\begin{split}
    P_{\epsilon} v^{\ep} 
    {:=} \frac{1}{r^2}
    \left(
    -\epsilon(v^{\ep}_{\xi \xi}+r v^{\ep}_{r}+r^{2}v^{\ep}_{r r} )-r^{2}\sin \xi v^{\ep}_{r}-r \cos \xi v^{\ep}_{\xi}+r^{2}(v^{\ep})^{3}
    \right)
    & =f \quad  \text{ in } D,\\
    v^{\ep}(1,\xi)&=0 \quad  \text{ at } 0 \leq \xi \leq 2\pi,
\end{split}
\end{equation}
where $D:=\{(r,\xi)| 0< r <1 , 0\leq \xi \leq 2\pi\}$.
For the sake of simplicity, we define the upper semi-circle as
$\Gamma_{+}:= \{ (x, y)|x^2 + y^2 = 1, y > 0\}$ and the lower semi-circle as $\Gamma_{-}:=\{ (x, y)|x^2 + y^2 = 1, y < 0\}$.
Performing the boundary layer analysis as in \cite{hong2014numerical}, we are led to the following equation for the corrector equation
\be \label{e:cor:circle}
\begin{split}
    - \ep \varphi^0_{rr} - (\sin \xi) \varphi^0_{r}  & = 0, \quad \text{  for  } 0 < r < 1, \quad 0 < \xi \leq 2 \pi, \\
     \varphi^0  & = - v^0(\cos \xi, \sin \xi), \quad \text{  on  } \Gamma_{-}, \\
     \varphi^0  & \rightarrow 0 \quad \text{ as } r \rightarrow 0.
\end{split}
\ee
Hence, we are able to find an explicit solution of the correction equation \eqref{e:cor:circle}:
\be
\varphi^0 = -v^0(\cos\xi \sin\xi)\exp\left(\frac{\sin \xi}{\ep} (1-r) \right) \chi_{\pi, 2\pi}(\xi),
\ee
where $\chi$ stands for the characteristic function.
To match the boundary condition in our numerical scheme, we introduce a cut-off function to derive an approximate form 
\be
\bar \varphi^0 = \exp\left(\frac{\sin \xi}{\ep} (1-r) \right) \chi_{\pi, 2\pi}(\xi) \delta(r),
\ee
where $\delta(r)$ is a smooth cut-off function such that $\delta(r) = 1$ for $r \in [3/4, 1]$ and $=0$ for $r \in [0, 1/2]$.
We now establish the semi-analytic SL-PINN method as
\begin{equation}\label{e:EPINN_scheme_circle01}
    \widetilde{v}(r,\xi ; \, {\blds \theta}) 
            =(\hat{v}(r,\xi, {\blds \theta})-\hat{v}(1,\xi, {\blds \theta}) {\bar \varphi^0})C(r,\xi),
\end{equation}
where $C(r,\xi)$ is given by
\begin{equation} \label{e:circle_C_term}
\begin{split}
    C(r,\xi)=\begin{cases}
    1-r^3 , \text{ if } 0 \leq \xi \leq \pi,\\
    1-r^3-(r\sin\xi)^3, \text{ if } \pi < \xi <2\pi,
    \end{cases}
\end{split}
\end{equation}
and $\hat{v}(r,\xi) = \hat{u}(x,y)$.
Then, the residual loss is defined by
\begin{equation} \label{e:circle_loss_first}
\begin{split}
    Loss=\frac{1}{N}\sum_{i=0}^{N} \| P_{\epsilon}\widetilde{v}((r_{i},\xi_{i}; {\blds \theta}))-f \|_{p} \quad  \text{ for }(r_{i},\xi_{i}) \in  D,
\end{split}    
\end{equation}
where $p=1,2$.
Since the boundary layer behavior occurs near the lower semi-circle, we divide the residual loss \eqref{e:circle_loss_first} into two parts: $0 \leq \xi \leq \pi$ and $\pi \leq \xi \leq 2 \pi$.
For the case of $0 \leq \xi \leq \pi$, the calculation of the residual loss is straightforward:
\begin{equation} \label{e:DD1c}
\begin{split}
    & P_{\epsilon}\widetilde{v}((r,\xi, {\blds \theta})) - f \\
    & =
    -\ep (\frac{1}{r^2}-r)\hat{v}_{\xi \xi}(r,\xi, {\blds \theta})+(r^2-\frac{1}{r}     )\cos(\xi)\hat{v}_{\xi}(r,\xi, {\blds \theta})-\ep(1-r^3)\hat{v}_{r r}(r,\xi, {\blds \theta}) \\
    & \qquad +(6\ep+\ep r^2-\frac{\ep}{r}-\sin(\xi)(1-r^3)      )\hat{v}_{r}(r,\xi, {\blds \theta})
    +(3\ep+\frac{6\ep}{r}+3 r^2 \sin(\xi)  )\hat{v}(r,\xi, {\blds \theta})-f,
\end{split}
\end{equation}




\begin{figure}[h!]
     \centering
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/circle_compatible_true_3d.png}
         \caption{True solution}
         %\label{fig:y equals x}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/circle_compatible_epinn_3d.png}
         \caption{SL-PINN using $L^2$ training}
         %\label{fig:y equals x}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/circle_compatible_epinn_3d_l1.png}
         \caption{SL-PINN using $L^1$ training}
         %\label{fig:three sin x}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/circle_compatible_pinn_3d.png}
         \caption{Conventional PINN}
         %\label{fig:three sin x}
     \end{subfigure}
             \caption{Numerical prediction of \eqref{e:circle_eq} with $\ep = 10^{-6}$ and $f=(1-x^2)^2$. For our simulations, we select a uniform grid of $50$ discretized points in each of the $\eta$ and $\tau$ directions.}\label{fig2}
\end{figure}

\begin{figure}[h!]
         \centering         \includegraphics[scale=0.4]{fig/true_vs_pred_circle_compatible_at_0.5pi.png}
         \caption{The one-dimensional profile of predicted solutions along the line $\tau = \pi/2$.}
\label{fig2-2}
\end{figure}






}



==> Convection_diffusion_on_elliptical.tex <==
\section{Convection-Diffusion Equations in an Elliptical Domain}
We explore the convection-diffusion equations on an elliptical domain, which represents a natural yet non-trivial extension of the problem:
\begin{equation} \label{e:ellipse}
\begin{split}
   L_{\epsilon}u^{\ep} {\color{red}:=}- \epsilon \Delta u^{\ep} - u^{\ep}_y & =f, \quad \text{  in  } \Omega=\left\{(x,y) | {\frac{x^{2}}{(R^{x})^{2}}}+\frac{y^{2}}{(R^{y})^{2}}< 1\right \}\\
     u^{\ep}  & = 0, \quad \text{  at  } \partial \Omega.
\end{split}    
\end{equation}
Within the elliptical domain, we utilize the elliptic coordinate system \cite{churchill1961mathematical} and examine two separate scenarios; \lowercase\expandafter{\romannumeral1}) $R^x > R^y$; \lowercase\expandafter{\romannumeral2}) $R^x < R^y$.\\ 


\subsection{Major Axis Parallel to \texorpdfstring{$x$-Axis}{x-Axis}}

%(\lowercase\expandafter{\romannumeral1}) $R^{x}>R^{y}$.
To start, we define the elliptic coordinates as $(\eta, \tau)$ such that
\begin{equation}
\begin{split}
    x=a\cosh (R-\eta) \cos \tau ,y=a\sinh (R-\eta) \sin \tau,
\end{split}
\end{equation}
where $\eta>0$ and $\tau \in [0, 2 \pi]$.
By setting $u^{\ep}(x,y)= v^{\ep}(\eta,\tau)$ with 
$$
a\cosh R =R^x, \quad
a\sinh R =R^y,
$$ \
we transform \eqref{e:ellipse} into the following form
\begin{equation}
\begin{split}
     P_{\epsilon} v^{\ep} {:=}-\epsilon(v^{\ep}_{\eta \eta}+v^{\ep}_{\tau \tau})+(a \cosh (R-\eta) \sin \tau)  v^{\ep}_{\eta}-(a\sinh (R-\eta) \cos \tau)v^{\ep}_{\tau} & = H f \quad \text{ in } D=[0,R)\times [0,2\pi]\\
      v^{\ep}(0,\tau)&=0 \text{ at } 0 \leq \tau \leq 2\pi,
\end{split}
\end{equation}
where $H=(a\sinh (R-\eta) \cos \tau )^{2}+(a \cosh (R-\eta) \sin \tau)^{2}$.
To derive the corrector equation of $\varphi$, we use the following stretching variable,
\begin{equation}
\begin{split}
    \overline{\eta}=&\frac{\eta}{\epsilon^{\alpha}}.
\end{split}
\end{equation}


\begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/slpinn_nonli_true.png}
        \caption{True solution}
         %\label{fig:y equals x}
    \end{subfigure}
     %\hfill
    \begin{subfigure}[b]{0.4\textwidth}
    \centering
        \includegraphics[width=\textwidth]{fig/slpinn_nonli_l2.png}
        \caption{SL-PINN using $L^2$ training}
         %\label{fig:y equals x}
    \end{subfigure}
     %\hfill
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/slpinn_nonli_l1.png}
        \caption{SL-PINN using $L^1$ training}
         %\label{fig:three sin x}
    \end{subfigure}
     %\hfill
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/slpinn_nonli_pinn.png}
        \caption{Conventional PINN}
         %\label{fig:three sin x}
    \end{subfigure}
        \caption{Numerical prediction of \eqref{e:circle_eq} with $\ep = 10^{-6}$ and $f=1+(u^{\epsilon})^{3}$, where $u$ is the solution of non-compatible case $f=1$ of \ref{e:circle_eq}.  For our simulations, we select a uniform grid of $50$ discretized points in each of the $\eta$ and $\tau$ directions.}\label{fig non-li}
\end{figure}






We then obtain the corrector equation with $\alpha = 1$, which is the thickness of the boundary layer, 
\begin{equation} \label{e:cor_elliptic_01}
\begin{split}
     -\varphi^0_{\overline{\eta \eta}}+& \left (a \left(\frac{e^{R-\epsilon\overline{\eta}}+e^{\epsilon\overline{\eta}-R}}{2} \right)\sin \tau \right) \varphi^0_{\overline{\eta}}=0.
\end{split}
\end{equation}
Instead of seeking an explicit solution for the corrector equation, we employ the Taylor series expansion for computational convenience to obtain a solution profile for \eqref{e:cor_elliptic_01},
\begin{equation} \label{e:cor_elliptic_02}
\begin{split}
     -\varphi^0_{\overline{\eta \eta}}+&\left(a
     \left(\frac{e^{R}+e^{-R}}{2}+\epsilon
     \left(\frac{e^{-R}-e^{R}}{2}\right)
     \overline{\eta}+\frac{\epsilon^{2}}{2!}
     \left(\frac{e^{R}+e^{-R}}{2}\right)
     \overline{\eta}^{2}+..          \right)
     \sin \tau\right) \varphi^0_{\overline{\eta}}=0.\\
\end{split}
\end{equation}
By identifying the dominant terms in equation \eqref{e:cor_elliptic_02}, we derive the approximate corrector equations,
\begin{equation}
\begin{split}
     -\varphi^0_{\overline{\eta \eta}}+
     \left(
     a
     \left(
     \frac{e^{R}+e^{-R}}{2}
     \right)
     \sin \tau
     \right)
     \varphi^0_{\overline{\eta}}=0,\\
     \varphi^0=-v^{0} \text{ at } \overline{\eta}=0.
\end{split}
\end{equation}
where $v^0(\eta,\tau) = u^0(x,y)$.
An explicit solution can be calculated as
\be \label{e:elliptic_cor}
     \bar{\varphi}^0(\overline{\eta},\tau)=-v^{0}(0,\tau) e^{(R^{x}\sin \tau) \overline{\eta}}.
\ee
For our numerical scheme, we introduce an approximate form,
\be
\bar \varphi^0 =\exp\left({\frac{R^{x}\sin\tau}{\varepsilon   }\eta}\right)\chi_{(\pi,2\pi)}\delta(\eta).
\ee
With \eqref{e:elliptic_cor}, we now introduce our {\it SL-PINN} of the form,
\begin{equation}\label{e:EPINN_scheme_ellipse01}
    \widetilde{v}(\eta,\tau ; \, {\blds \theta}) 
            =
            \left(\hat{v}(\eta,\tau,{\blds \theta})-\hat{v}(0,\tau,{\blds \theta})
            {\bar \varphi^0(\eta,\tau)}\right)C(\eta,\tau),
\end{equation}
where $C(\eta,\tau)$ is the regularizing term given by
\begin{equation} \label{e:ellipse_reg01}
\begin{split}
    C(\eta,\tau)=\begin{cases}
    1-\left(\frac{R-\eta}{R}\right)^{3} , \text{ if } 0 \leq \tau \leq \pi\\
    1-\left(\frac{R-\eta}{R}\right)^{3}-\left(\frac{R-\eta}{R}\sin\tau \right)^3, \text{ if } \pi < \tau <2\pi.
    \end{cases}
\end{split}
\end{equation} 
Then, the residual loss is defined by
\begin{equation} \label{e:ellipse_loss_first}
\begin{split}
    Loss=\frac{1}{N}\sum_{i=0}^{N}
    \|P_{\epsilon}\widetilde{v}((\eta_{i},\tau_{i},{\blds \theta}))-f \|_{p} \quad  \text{ for }(\eta_{i},\tau_{i}) \in D,
\end{split}    
\end{equation} 
where $p=1,2$. To account for the boundary layer behavior occurring near the boundary where $\pi \leq \tau \leq 2 \pi$, we divide the residual loss \eqref{e:ellipse_loss_first} into two sections: $0 \leq \tau \leq \pi$ and $\pi \leq \tau \leq 2 \pi$. Calculating the residual loss is straightforward for the range of $0 \leq \tau \leq \pi$:
\begin{equation} \label{x_upper_elipse_cal}
\begin{split}
    &P_{\epsilon}\widetilde{v}(\eta,\tau,{\blds \theta}) - f \\
    & = -\ep \left( \hat{v}_{\eta \eta}(\eta,\tau,{\blds \theta}) \left(1 - \left(\frac{R-\eta}{R}\right)^3\right) - 2\hat{v}_{\eta}(\eta,\tau,{\blds \theta}) \left(-3 \frac{(R-\eta)^2}{R^3}\right) + \hat{v}(\eta,\tau,{\blds \theta}) \left(-6 \frac{R-\eta}{R^3}\right) \right. \\
    & \quad + \left. \hat{v}_{\tau \tau}(\eta,\tau,{\blds \theta}) \left(1 - \left(\frac{R-\eta}{R}\right)^3\right) \right) \\
    & \quad - (a \cosh (R-\eta) \sin \tau) \left( \hat{v}_{\eta}(\eta,\tau,{\blds \theta}) \left(1 - \left(\frac{R-\eta}{R}\right)^3\right) + \hat{v}(\eta,\tau,{\blds \theta}) \left(-3 \frac{(R-\eta)^2}{R^3}\right) \right) \\
    & \quad - (a \sinh (R-\eta) \cos \tau) \hat{v}_{\tau}(\eta,\tau,{\blds \theta}) \left(1 - \left(\frac{R-\eta}{R}\right)^3\right) - f \\
    & \text{for } 0 < \eta \leq R \;, 0 \leq \tau \leq \pi.
\end{split}
\end{equation}






However, when considering $\pi \leq \tau \leq 2 \pi$, incorporating the boundary layer element in \eqref{e:EPINN_scheme_ellipse01} and including the regularizing term in \eqref{e:ellipse_reg01} result in a more intricate form of the residual loss, as shown below:
\begin{equation} \label{x_lower_elipse_cal}
\begin{split}
    &P_{\epsilon}\widetilde{v}(\eta,\tau,{\blds \theta}) - f = \\
    &-\ep \left( \hat{v}_{\eta \eta}(\eta,\tau,{\blds \theta})C + 2\hat{v}_{\eta}(\eta,\tau,{\blds \theta})C_{\eta} + \hat{v}(\eta,\tau,{\blds \theta})C_{\eta \eta} + \hat{v}_{\tau \tau}(\eta,\tau,{\blds \theta})C + 2\hat{v}_{\tau}(\eta,\tau,{\blds \theta})C_{\tau} + \hat{v}(\eta,\tau,{\blds \theta})C_{\tau \tau} \right) \\
    &+(a \cosh (R-\eta) \sin \tau) \left( \hat{v}_{\eta}(\eta,\tau,{\blds \theta})C + \hat{v}(\eta,\tau,{\blds \theta})C_{\eta} \right) \\
    &-(a \sinh (R-\eta) \cos \tau) \left( \hat{v}_{\tau}(\eta,\tau,{\blds \theta})C + \hat{v}(\eta,\tau,{\blds \theta})C_{\tau} \right) \\
    &+\ep \hat{v}(0,\tau,{\blds \theta}) \left[ \delta_{\eta \eta}C + 2 \delta_{\eta}C_{\eta} + \delta C_{\eta \eta} \right] \exp\left( \frac{R^{x} \sin \tau}{\ep} \eta \right) \\
    &+\hat{v}(0,\tau,{\blds \theta}) \left[ 2R^{x} \sin \tau \delta_{\eta}C + 2R^{x} \sin \tau \delta C_{\eta} \right] \exp\left( \frac{R^{x} \sin \tau}{\ep} \eta \right) \\
    &+a (\cosh (R-\eta) \sin \tau) \hat{v}(0,\tau,{\blds \theta}) \left[ \delta_{\eta} C + \delta C_{\eta} \right] \exp\left( \frac{R^{x} \sin \tau}{\ep} \eta \right) \\
    &+\ep \delta \left[ \hat{v}_{\tau \tau}(\eta,\tau,{\blds \theta})C + 2\hat{v}_{\tau}(\eta,\tau,{\blds \theta})C_{\tau} + \hat{v}(\eta,\tau,{\blds \theta})C_{\tau \tau} \right] \exp\left( \frac{R^{x} \sin \tau}{\ep} \eta \right) \\
    &-\delta \left[ R^{x} \eta \left( (\sin \tau \hat{v}(\eta,\tau,{\blds \theta}) - 2\cos \tau \hat{v}_{\tau}(\eta,\tau,{\blds \theta}))C - 2(\cos \tau \hat{v}(\eta,\tau,{\blds \theta}))C_{\tau} \right) \right] \exp\left( \frac{R^{x} \sin \tau}{\ep} \eta \right) \\
    &+\frac{\hat{v}(0,\tau,{\blds \theta})}{\ep} \delta C \left[ (R^{x} \sin \tau)^{2} - a \cosh (R-\eta) \sin^2 \tau R^{x} + (R^{x}\eta \cos \tau)^{2} + a \sinh (R-\eta) \cos^2 \tau R^{x} \eta \right]\\ 
    &\times \exp\left( \frac{R^{x} \sin \tau}{\ep} \eta \right) - f \\
    & \text{for } 0 < \eta \leq R \;, \pi \leq \tau \leq 2\pi.
\end{split}
\end{equation}



As in the circular domain, calculating the residual loss in \eqref{x_lower_elipse_cal} involves a substantial term that can misguide our loss optimization process. 
In order to make the computation in equation \eqref{x_lower_elipse_cal} feasible, we extract the dominant term in $\ep$, specifically the term of $\mathcal{O}(\ep^{-1})$. This allows us to derive
{\color{red}
\begin{equation}
\begin{split} 
    \psi(\eta,\tau,{\blds \theta}):=\frac{\hat{v}(0,\tau,{\blds \theta})}{\ep}\delta(\eta) (1-(\frac{R-\eta}{R})^{3}-(\frac{R-\eta}{R}\sin\tau)^3)[(R^{x}\sin\tau)^{2}-a\cosh (R-\eta)\sin^2\tau R^{x}\\
    +(R^{x}\eta\cos\tau)^{2}+a\sinh (R-\eta) \cos^2\tau R^{x}\eta]
    \exp\left( \frac{R^{x}\sin \tau}{\ep} \eta \right).
\end{split}
\end{equation}





\noindent\textbf{Remark 5.1.} It holds that
\[
    \left\| \frac{1}{\epsilon} \exp\left( \frac{R^{x} \sin \tau}{\epsilon} \eta \right) \right\|_{L^{1}(D^{*})} < C_{1},
\]
where \(C_{1}, C_{2}\) are constants.



By the triangular inequality, the loss in \eqref{e:ellipse_loss_first} bounds
\begin{equation}\label{e:bound_ellipse00}
 Loss  \leq \frac{1}{N}\sum_{i=0}^{N}|\psi (\eta_{i},\tau_{i},{\blds \theta})|
 +  \frac{1}{N}\sum_{i=0}^{N} |P_{\epsilon}\widetilde{v}((\eta_{i},\tau_{i},{\blds \theta}))-\psi (\eta_{i},\tau_{i},{\blds \theta})-f|,
\end{equation}
The rightmost term does not involve a high-order term, such as ${\ep^{\alpha}}$ where $\alpha < 0$, as $\psi$ already contains large terms like $\ep^{-1}$. Therefore, this part can be computed using a conventional $L^1$ or $L^2$ loss. Considering that $\psi$ contains terms of $\mathcal{O}(\epsilon^{-1})$, we utilize an $L^1$ loss for handling $\psi$. To ensure accuracy, we select a sufficiently large number of sampling points, denoted as $N$:
\begin{equation}\label{e:bound_ellipse01}
\begin{split}
     & \frac{1}{N}\sum_{i=0}^{N} \left|\psi(\eta_{i},\tau_{i},{\blds \theta}) \right| \approx \frac{1}{R\pi}\int^{2\pi}_{\pi} \int^{R}_{0} |\psi(\eta,\tau,{\blds \theta})|d \eta d \tau\\
\end{split}
\end{equation}

\begin{comment}
    Note that, $\delta(r)$ is a smooth cut-off function such that $\delta(r) = 1$ for $r \in [3R/4 , R]$ and $=0$ for $r \in [0, R/2]$.
\end{comment}


The right-hand side of equation (\ref{e:bound_ellipse01}) is bounded by \(C_1 \), by using the Remark 5.1. Particularly, we obtain:



\begin{equation}\label{e:bound_ellipse02}
\begin{split}
    \frac{1}{R\pi}&\int^{2\pi}_{\pi}\int^{R}_{0} |P_{\epsilon}\psi(\eta,\tau,{\blds \theta})|d \eta d \tau\\
    & \leq K\pi(R^{x}+a\cosh R)(1-e^{-R^{x}R/ 2\ep})+\frac{1}{4}KR^{x}R^{2}+2Ka(\cosh{R}-\cosh(R/2)).
\end{split}
\end{equation}}


Thus, in \eqref{e:bound_ellipse00}, we focus on minimizing the rightmost term, as the first term on the right-hand side of \eqref{e:bound_ellipse00} becomes nearly constant by \eqref{e:bound_ellipse02} when $\ep$ is sufficiently small.
This simplification enables feasible computations in our analysis.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/ellipse_y_true_3d.png}
         \caption{True solution}
         %\label{fig:y equals x}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/ellipse_y_lspinn_3d.png}
         \caption{SL-PINN using $L^2$ training}
         %\label{fig:three sin x}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/ellipse_y_lspinn_3d_l1.png}
         \caption{SL-PINN using $L^1$ training}
         %\label{fig:three sin x}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/ellipse_y_pinn_3d.png}
         \caption{Conventional PINN}
         %\label{fig:three sin x}
     \end{subfigure}
     \caption{Numerical prediction of \eqref{e:ellipse} with $(R^x,R^y)=(4,1)$ and $\ep = 10^{-6}$ when $f={(1-({x}/{R^x})^2)^2}/{R^y}$. For our simulations, we select a uniform grid of $50$ discretized points in each of the $r$ and $\tau$ directions.} \label{fig6}
\end{figure}









\begin{figure}%[htbp]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/true_vs_pred_ellipse_y_at_0.5pi.png}
        \caption{True soltuion at t=1}
         %\label{fig:y equals x}
    \end{subfigure}
     %\hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/X_major_2d.png}
        \caption{SL-PINN}
         %\label{fig:three sin x}
    \end{subfigure}
    \caption{The one-dimensional profile of predicted solutions in Figure \ref{fig6} along the line $\tau = \pi/2$ and solution surface projection profile.}\label{fig6-6}
\end{figure}



\begin{comment}
\begin{figure}%[htbp]
         \centering
             \includegraphics[trim={0 3cm 0 3cm},clip,scale=0.5]{fig/true_vs_pred_ellipse_y_at_0.5pi.png}
         \caption{The one-dimensional profile of predicted solutions in Figure \ref{fig6} along the line $\tau = \pi/2$.}\label{fig6-6}
\end{figure}
\end{comment}


The effectiveness of our new approach is demonstrated through a series of numerical experiments presented in Figures (\ref{fig6}) and (\ref{fig6-6}). In these experiments, we utilize a grid discretization consisting of $50$ uniformly spaced points in both the $\tau$ and $r$ directions.
Similar to the circular domain, when $f$ does not vanish at the characteristic points $(\pm 4, 0)$  the function $f(x, y)$ becomes incompatible due to the appearance of singularities in its derivatives at these points.
To maintain simplicity in this paper, we focus on the first compatibility condition.
We compare the performance of the standard five-layer PINN approximation with our SL-PINN approximation. Figure \ref{fig6} showcases the numerical solutions of \eqref{e:ellipse} with $(R^x,R^y)=(4,1)$ and $\ep = 10^{-6}$ when $f={(1-({x}/{R^x})^2)^2}/{R^y}$.
Figure \ref{fig6} provides a clear illustration of the conventional PINN method's failure in accurately approximating the solution to the singular perturbation problem.
In contrast, our new scheme exhibits significant superiority over the conventional PINN method. The numerical results presented in Figure \ref{fig6} and Table \ref{tab:1} provide compelling evidence of the substantial performance improvement achieved by our SL-PINN approach. Our semi-analytic SL-PINN, enriched with the corrector, consistently produces stable and accurate approximate solutions regardless of the small parameter $\ep$.
Figure \ref{fig6-6} offers a closer examination of the one-dimensional profile of predicted solutions at $\tau=\pi/2$, facilitating a clear and direct comparison. Figure \ref{fig6-6} vividly demonstrates the high accuracy of both the $L^1$ and $L^2$ training approaches in generating approximations. However, the conventional PINN method falls short in capturing the sharp transition near the boundary layer.




\subsection{Major Axis Parallel to \texorpdfstring{$y$-Axis}{y-Axis}}

We now define the elliptic coordinates as $(\eta, \tau)$ such that
\begin{equation}
\begin{split}
    x=a\sinh (R-\eta) \cos \tau ,y=a\cosh (R-\eta) \sin \tau,
\end{split}
\end{equation}
where $r>0$ and $\tau \in [0, 2 \pi]$.
Setting $u^{\ep}(x,y)= v^{\ep}(\eta,\tau)$ and  $a\sinh R =R^x,$ and $a\cosh R =R^y$, we transform \eqref{e:ellipse} into the following form
\begin{equation}
\begin{split}
     P_{\epsilon} v^{\ep} :=-\epsilon(v^{\ep}_{\eta \eta}+v^{\ep}_{\tau \tau})+(a \sinh (R-\eta) \sin \tau)  v^{\ep}_{\eta}-(a\cosh (R-\eta) \cos \tau)v^{\ep}_{\tau} & = H f \quad \text{ in } D=[0,R)\times [0,2\pi]\\
      v^{\ep}(0,\tau)&=0 \text{ at } 0 \leq \tau \leq 2\pi,
\end{split}
\end{equation}
where $H=(a\sinh (R-\eta) \sin \tau )^{2}+(a \cosh (R-\eta) \cos \tau)^{2}$.
To derive the corrector equation of $\varphi$, we make use of the following stretching variable,
\begin{equation}
\begin{split}
    \overline{\eta}=&\frac{\eta}{\epsilon^{\alpha}}.
\end{split}
\end{equation}
We then obtain the corrector equation with $\alpha = 1$, which is the thickness of the boundary layer, 
\begin{equation} \label{e:cor_elliptic}
\begin{split}
     -\varphi^0_{\overline{\eta \eta}}+& \left (a \left(\frac{e^{R-\epsilon\overline{\eta}}-e^{\epsilon\overline{\eta}-R}}{2} \right)\sin \tau \right) \varphi^0_{\overline{\eta}}=0.
\end{split}
\end{equation}
To find an explicit solution for the corrector, we simplify \eqref{e:cor_elliptic} by applying the Taylor series expansion,
\begin{equation}\label{e:cor_elliptic_02_y}
\begin{split}
     -\varphi^0_{\overline{\eta \eta}}+&\left(a
     \left(\frac{e^{R}-e^{-R}}{2}-\epsilon
     \left(\frac{e^{-R}+e^{R}}{2}\right)
     \overline{\eta}+\frac{\epsilon^{2}}{2!}
     \left(\frac{e^{R}-e^{-R}}{2}\right)
     \overline{\eta}^{2}-..          \right)
     \sin \tau\right) \varphi^0_{\overline{\eta}}=0.\\
\end{split}
\end{equation}
By identifying the dominant terms in equation \eqref{e:cor_elliptic_02_y}, we derive the approximate corrector equations,
\begin{equation}
\begin{split}
     -\varphi^0_{\overline{\eta \eta}}+
     \left(
     a
     \left(
     \frac{e^{R}-e^{-R}}{2}
     \right)
     \sin \tau
     \right)
     \varphi^0_{\overline{\eta}}=0\\
     \varphi^0=-v^{0} \text{ at } \overline{\eta}=0,
\end{split}
\end{equation}
where $v^0(\eta,\tau) = u^0(x,y)$.
An explicit solution can be calculated as
\be\label{e:elliptic_y_cor}
     \bar{\varphi}^0(\overline{\eta},\tau)=-v^{0}(0,\tau) e^{(R^{x}\sin \tau) \overline{\eta}}.
\ee
{For our numerical scheme, we introduce an approximate form,
\be
\bar \varphi^0 =\exp\left({\frac{R^{x}\sin\tau}{\varepsilon   }\eta}\right)\tau_{(\pi,2\pi)}\delta(\eta).
\ee}
With \eqref{e:elliptic_y_cor}, we now introduce our {\it SL-PINN} of the form,
\begin{equation}\label{e:EPINN_scheme_ellipse02}
    \widetilde{v}(\eta,\tau ; \, {\blds \theta}) 
            =
            \left(\hat{v}(\eta,\tau,{\blds \theta})-\hat{v}(0,\tau,{\blds \theta})
            {\bar \varphi^0}\right)C(\eta,\tau),
\end{equation}
where $C(\eta,\tau)$ is the boundary regularizing term given by
\begin{equation} \label{e:ellipse_reg02}
\begin{split}
    C(\eta,\tau)=\begin{cases}
    1-(\frac{R-\eta}{R})^{3} , \text{ if } 0 \leq \tau \leq \pi,\\
    1-(\frac{R-\eta}{R})^{3}-(\frac{R-\eta}{R}\sin\tau)^3, \text{ if } \pi < \tau <2\pi.
    \end{cases}
\end{split}
\end{equation}
Then, the residual loss is defined by
\begin{equation}\label{e:ellipse_loss_second}
\begin{split}
    Loss=\frac{1}{N}\sum_{i=0}^{N}\|P_{\epsilon}\widetilde{v}((\eta_{i},\tau_{i},{\blds \theta}))-f \|_{p} \quad  \text{ for }(\eta_{i},\tau_{i}) \in D,
\end{split}    
\end{equation}
where $p=1,2$. 
Considering the boundary layer behavior near $\pi \leq \tau \leq 2 \pi$, we split the residual loss  \eqref{e:ellipse_loss_second} into two sections: $0 \leq \tau \leq \pi$ and $\pi \leq \tau \leq 2 \pi$. 
The residual loss calculation for $0 \leq \tau \leq \pi$ is relatively simple:

\begin{equation}\label{y-upper-elipse}
\begin{split}
    &P_{\epsilon}\widetilde{v}((R-\eta,\tau,{\blds \theta})) - f = \\
    &-\ep \left( \hat{v}_{\eta \eta}(\eta,\tau,{\blds \theta}) \left(1 - \left(\frac{R-\eta}{R}\right)^3\right) - 2\hat{v}_{\eta}(\eta,\tau,{\blds \theta}) \left(-3 \frac{(R-\eta)^2}{R^3}\right) + \hat{v}(\eta,\tau,{\blds \theta}) \left(-6 \frac{R-\eta}{R^3}\right) \right. \\
    & \quad + \left. \hat{v}_{\tau \tau}(\eta,\tau,{\blds \theta}) \left(1 - \left(\frac{R-\eta}{R}\right)^3\right) \right) \\
    &+(a \sinh (R-\eta) \sin \tau) \left( \hat{v}_{\eta}(\eta,\tau,{\blds \theta}) \left(1 - \left(\frac{R-\eta}{R}\right)^3\right) + \hat{v}(\eta,\tau,{\blds \theta}) \left(3 \frac{(R-\eta)^2}{R^3}\right) \right) \\
    &-(a \cosh (R-\eta) \cos \tau) \hat{v}_{\tau}(\eta,\tau,{\blds \theta}) \left(1 - \left(\frac{R-\eta}{R}\right)^3\right) - f,
\end{split}
\end{equation}
for $0 < \eta \leq R \;, 0 \leq \tau \leq \pi$.


However, when considering $\pi \leq \tau \leq 2 \pi$, incorporating the boundary layer element in \eqref{e:EPINN_scheme_ellipse02} and including the regularizing term in \eqref{e:ellipse_reg02} result in a more intricate form of the residual loss, as shown below:


\begin{equation}\label{y-lower-elipse}
\begin{split}
    &P_{\epsilon}\widetilde{v}((R-\eta,\tau,{\blds \theta})) - f = \\
    &-\ep \left( \hat{v}_{\eta \eta}(\eta,\tau,{\blds \theta})C + 2\hat{v}_{\eta}(\eta,\tau,{\blds \theta})C_{\eta} + \hat{v}(\eta,\tau,{\blds \theta})C_{\eta \eta} + \hat{v}_{\tau \tau}(\eta,\tau,{\blds \theta})C + 2\hat{v}_{\tau}(\eta,\tau,{\blds \theta})C_{\tau} + \hat{v}(\eta,\tau,{\blds \theta})C_{\tau \tau} \right) \\
    &+(a \sinh (R-\eta) \sin \tau) \left( \hat{v}_{\eta}(\eta,\tau,{\blds \theta})C + \hat{v}(\eta,\tau,{\blds \theta})C_{\eta} \right) \\
    &-(a \cosh (R-\eta) \cos \tau) \left( \hat{v}_{\tau}(\eta,\tau,{\blds \theta})C + \hat{v}(\eta,\tau,{\blds \theta})C_{\tau} \right) \\
    &+\ep \hat{v}(0,\tau,{\blds \theta}) \left[ \delta_{\eta \eta}C + 2 \delta_{\eta}C_{\eta} + \delta C_{\eta \eta} \right] \exp\left( \frac{R^{x}\sin \tau}{\ep} \eta \right) \\
    &+\hat{v}(0,\tau,{\blds \theta}) \left[ 2R^{x} \sin \tau \delta_{\eta}C + 2R^{x} \sin \tau \delta C_{\eta} \right] \exp\left( \frac{R^{x}\sin \tau}{\ep} \eta \right) \\
    &-a (\cosh (R-\eta) \sin \tau) \hat{v}(0,\tau,{\blds \theta}) \left[ \delta_{\eta} C + \delta C_{\eta} \right] \exp\left( \frac{R^{x} \sin \tau}{\ep} \eta \right) \\
    &+\ep \delta \left[ \hat{v}_{\tau \tau}(\eta,\tau,{\blds \theta})C + 2\hat{v}_{\tau}(\eta,\tau,{\blds \theta})C_{\tau} + \hat{v}(\eta,\tau,{\blds \theta})C_{\tau \tau} \right] \exp\left( \frac{R^{x} \sin \tau}{\ep} \eta \right) \\
    &-\delta \left[ R^{x} \eta \left( (\sin \tau \hat{v}(\eta,\tau,{\blds \theta}) - 2\cos \tau \hat{v}_{\tau}(\eta,\tau,{\blds \theta}))C - 2(\cos \tau \hat{v}(\eta,\tau,{\blds \theta}))C_{\tau} \right) \right] \exp\left( \frac{R^{x} \sin \tau}{\ep} \eta \right) \\
    &+\frac{\hat{v}(0,\tau,{\blds \theta})}{\ep} \delta C \left[ (R^{x} \sin \tau)^{2} - a \sinh (R-\eta) \sin^2 \tau R^{x} + (R^{x}\eta \cos \tau)^{2} + a \cosh (R-\eta) \cos^2 \tau R^{x}\eta \right]\\
    &\times \exp\left( \frac{R^{x} \sin \tau}{\ep} \eta \right) - f,
\end{split}
\end{equation}
for $0 < \eta \leq R \;, \pi \leq \tau \leq 2\pi$.

Similar to the circular domain, the residual loss indicated in \eqref{x_lower_elipse_cal} encompasses a substantial term that may potentially misdirect our loss optimization process.
In order to make the computation in \eqref{x_lower_elipse_cal} feasible, we extract the dominant term in $\epsilon$, specifically the term of $\mathcal{O}(\epsilon^{-1})$.
Hence, we define
\begin{equation}
\begin{split} 
    \psi(\eta,\tau,{\blds \theta}):=\frac{\hat{v}(0,\tau,{\blds \theta})}{\ep}\delta(\eta) (1-(\frac{R-\eta}{R})^{3}-(\frac{R-\eta}{R}\sin\tau)^3)[(R^{x}\sin\tau)^{2}-a\sinh (R-\eta)\sin^2\tau R^{x}\\
    +(R^{x}\eta\cos\tau)^{2}+a\cosh (R-\eta) \cos^2\tau R^{x}\eta]
    \exp\left( \frac{R^{x}\sin \tau}{\ep} \eta \right).
\end{split}
\end{equation}
By the triangular inequality, the loss in \eqref{e:ellipse_loss_second} bounds
\begin{equation}\label{e:bound_ellipse000}
 Loss  \leq \frac{1}{N}\sum_{i=0}^{N}|\psi (\eta_{i},\tau_{i},{\blds \theta})|
 +  \frac{1}{N}\sum_{i=0}^{N} |P_{\epsilon}\widetilde{v}((\eta_{i},\tau_{i},{\blds \theta}))-\psi (\eta_{i},\tau_{i},{\blds \theta})-f|.
\end{equation}
Since $\psi$ absorbs large terms such as $\epsilon^{-1}$, the rightmost term does not involve high-order terms such as ${\epsilon^{\alpha}}$ where $\alpha < 0$. 
Given that $\psi$ includes terms of $\mathcal{O}(\epsilon^{-1})$, we employ an $L^1$ loss function for managing $\psi$:
\begin{equation}
\begin{split}
     & \frac{1}{N}\sum_{i=0}^{N}|\psi(\eta_{i},\tau_{i},{\blds \theta})| \approx \frac{1}{R\pi}\int^{2\pi}_{\pi} \int^{R}_{0} |\psi(\eta,\tau,{\blds \theta})|d \eta d \tau,
\end{split}
\end{equation}
where $N$ is the number of sampling points.

The right-hand side of equation (5.17) is bounded by \(C_1 \), as noted by the remark. Particularly, we can get:

By employing calculations similar to those presented in equations \eqref{e:bound_ellipse00} to \eqref{e:bound_ellipse02}, we can deduce the following result:
\begin{equation}\label{e:bound_ellipse020}
\begin{split}
     &\frac{1}{R\pi}\int^{2\pi}_{\pi} \int^{R}_{0} |\psi(\eta,\tau,{\blds \theta})|d \eta d \tau\\
    & \leq K \pi(R^{x}+a\sinh R)(1-e^{-R^{x}R/ 2\ep})+\frac{1}{4}KR^{x}R^{2}+2Ka(\sinh{R}-\cosh(R/2)).
\end{split}
\end{equation}


\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/ellipse_x_true_3d.png}
         \caption{True solution}
         %\label{fig:y equals x}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/ellipse_x_epinn_3d.png}
         \caption{SL-PINN using $L^2$ training}
         %\label{fig:y equals x}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/ellipse_x_epinn_3d_l1.png}
         \caption{SL-PINN using $L^1$ training}
         %\label{fig:y equals x}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/ellipse_x_pinn_3d.png}
         \caption{Conventional PINN}
         %\label{fig:three sin x}
     \end{subfigure}
     %\hfill
     \caption{Numerical prediction of \eqref{e:ellipse} with $(R^x,R^y)=(1,4)$ and $\ep = 10^{-6}$ when $f={(1-({x}/{R^x})^2)^2}/{R^y}$. For our simulations, we select a uniform grid of $50$ discretized points in each of the $r$ and $\tau$ directions.}\label{fig7-0}
\end{figure}






\begin{figure}%[htbp]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/true_vs_pred_ellipse_x_at_0.5pi.png}
        \caption{True soltuion at t=1}
         %\label{fig:y equals x}
    \end{subfigure}
     %\hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/Y_major_2d.png}
        \caption{SL-PINN}
         %\label{fig:three sin x}
    \end{subfigure}
    \caption{The one-dimensional profile of predicted solutions in Figure \ref{fig7-0} along the line $\tau = \pi/2$ and solution surface projection profile.}\label{fig7}
\end{figure}


\begin{comment}

\begin{figure}%[htbp]
         \centering
         \includegraphics[trim={1cm 4cm 1cm 4cm},clip,scale=0.5]{fig/true_vs_pred_ellipse_x_at_0.5pi.png}
        \caption{The one-dimensional profile of predicted solutions in Figure \ref{fig7-0} along the line $\tau = \pi/2$.}\label{fig7}
\end{figure}
\end{comment}

\begin{table}[htbp]




\begin{tabular}{ |p{1.8cm}|p{1.8cm}|p{1.8cm}|p{1.8cm}|p{1.8cm}|p{1.8cm}|p{1.8cm}|p{1.8cm}| }
 \hline
 \multicolumn{8}{|c|}{Relative $L^2$ error by the $L^2$ training (PINN)} \\
 \hline
    & square (Fig. \ref{fig1})& circle with non compatible (Fig. \ref{fig3}) & circle with compatible (Fig. \ref{fig2}) & ellipse 4:1 (Fig. \ref{fig6})& ellipse 1:4 (Fig. \ref{fig7-0})& oscillation (Fig. \ref{fig4}) & non-linear case (Fig. \ref{fig non-li}) \\
 \hline
 $\epsilon=10^{-4}$   & $9.55\times10^{-1}$    &$9.20\times10^{-1}$ &  $9.27\times10^{-1}$&  $8.55\times10^{-1}$&  $7.84\times10^{-1}$&  $8.76\times10^{-1}$&  $2.90\times10^{-1}$ \\
 $\epsilon=10^{-6}$&   $9.55\times10^{-1}$  & $9.21\times10^{-1}$   &$9.27\times10^{-1}$ &$8.65\times10^{-1}$&  $7.03\times10^{-1}$&  $9.12\times10^{-1}$&  $6.11\times10^{-1}$ \\
  $\epsilon=10^{-8}$ & $9.55\times10^{-1}$&$9.15\times10^{-1}$ &$9.20\times10^{-1}$ &  $8.62\times10^{-1}$ &  $7.85\times10^{-1}$ &  $9.23\times10^{-1}$ &  $4.13\times10^{-1}$ \\
 \hline
\end{tabular}










\begin{tabular}{ |p{1.8cm}|p{1.8cm}|p{1.8cm}|p{1.8cm}|p{1.8cm}|p{1.8cm}|p{1.8cm}|p{1.8cm}| }
 \hline
 \multicolumn{8}{|c|}{Relative $L^2$ error by $L^2$ training (SL-PINN)} \\
 \hline
 & square (Fig. \ref{fig1})& circle with non compatible (Fig. \ref{fig3}) & circle with compatible (Fig. \ref{fig2}) & ellipse 4:1 (Fig. \ref{fig6})& ellipse 1:4 (Fig. \ref{fig7-0})& oscillation (Fig. \ref{fig4})& non-linear case (Fig. \ref{fig non-li}) \\
 \hline
 $\epsilon=10^{-4}$   & $2.5\times10^{-3}$    &$3.2\times10^{-3}$ &  $1.6\times10^{-3}$&  $5.1\times10^{-3}$&  $2.6\times10^{-3}$&  $6.5\times10^{-3}$&  $4.2\times10^{-3}$ \\
 $\epsilon=10^{-6}$&   $2.0\times10^{-3}$  & $2.8\times10^{-3}$   &$1.5\times10^{-3}$ &$3.9\times10^{-3}$&  $1.7\times10^{-3}$&  $7.6\times10^{-3}$&  $3.5\times10^{-3}$ \\
  $\epsilon=10^{-8}$ & $2.0\times10^{-3}$   &$4.7\times10^{-3}$ &$2.3\times10^{-3}$ &  $5.8\times10^{-3}$ &  $2.8\times10^{-3}$ &  $9.5\times10^{-3}$&  $5.0\times10^{-3}$ \\
 \hline
\end{tabular}

\begin{tabular}{ |p{1.8cm}|p{1.8cm}|p{1.8cm}|p{1.8cm}|p{1.8cm}|p{1.8cm}|p{1.8cm}|p{1.8cm}|  }
 \hline
 \multicolumn{8}{|c|}{Relative $L^2$ error by $L^1$ training (SL-PINN)} \\
 \hline
 & square (Fig. \ref{fig1})& circle with non compatible (Fig. \ref{fig3}) & circle with compatible (Fig. \ref{fig2}) & ellipse 4:1 (Fig. \ref{fig6})& ellipse 1:4 (Fig. \ref{fig7-0})& oscillation (Fig. \ref{fig4})& non-linear case (Fig. \ref{fig non-li}) \\
 \hline
 $\epsilon=10^{-4}$   & $9.5\times10^{-5}$    &$4.2\times10^{-3}$ &  $2.6\times10^{-3}$&  $2.3\times10^{-3}$&  $3.4\times10^{-3}$&  $4.0\times10^{-2}$&  $3.5\times10^{-3}$ \\
 $\epsilon=10^{-6}$&   $1.4\times10^{-4}$  & $3.6\times10^{-3}$   &$4.6\times10^{-3}$ &$5.6\times10^{-3}$&  $4.2\times10^{-3}$&  $5.2\times10^{-2}$&  $4.0\times10^{-3}$ \\
  $\epsilon=10^{-8}$ & $3.9\times10^{-4}$   &$4.3\times10^{-3}$ &$1.8\times10^{-3}$ &  $3.4\times10^{-3}$ &  $4.8\times10^{-3}$ &  $6.2\times10^{-2}$ &  $5.0\times10^{-3}$ \\
 \hline
\end{tabular}





\caption{Comparison of relative $L^2$ errors for equations \eqref{e:square}, \eqref{e:circle_eq}, and \eqref{e:ellipse} utilizing standard 5-layer PINN, SL-PINN employing $L^2$ training, and SL-PINN employing $L^1$ training.} \label{tab:1}
\end{table}



\noindent
Hence, in \eqref{e:bound_ellipse000}, we focus on minimizing the rightmost term, since the first term on the right-hand side of \eqref{e:bound_ellipse000} becomes nearly constant by \eqref{e:bound_ellipse020} when $\ep$ is sufficiently small.
This simplification enables feasible computations in our computation.
Figures (\ref{fig7-0}) provide numerical evidence of the SL-PINN's effectiveness. For these experiments, we employed a grid comprising 50 uniformly spaced points in both the $\tau$ and $\eta$ directions.
We compare the standard five-layer PINN with our SL-PINN. 
Figure \ref{fig7-0} shows the numerical solutions of \eqref{e:ellipse} with $(R^x,R^y)=(1,4)$ and $\ep = 10^{-6}$ when $f={(1-({x}/{R^x})^2)^2}/{R^y}$. The figure underscores the traditional PINN's inability to accurately approximate the solution to the singular perturbation problem. In contrast, our novel approach demonstrates superior performance.
Figure \ref{fig7} offers a detailed view of the one-dimensional profile of predicted solutions at $\tau=\pi/2$. This demonstrates the high accuracy of both the $L^1$ and $L^2$ training approaches in predicting solutions. However, the traditional PINN method falls short in capturing the sharp transition near the boundary layer.


% {\color{gray} 
% To increase the expressive power of EPINN, we set up a 4-layer neural network such that
% \begin{equation}\label{e:NN}
%     \hat{u}({{x,y}}; \, {\blds \theta})
%     =
% W_5\sigma(W_4\sigma(W_3\sigma(W_1 x+W_2 y+b)+b)), 
% \end{equation}
% We now establish the semi-analytic enriched PINN method as
% \begin{equation}\label{e:EPINN_scheme_circle}
%     \widetilde{v}(r,\xi ; \, {\blds \theta}) 
%             =(\hat{v}(r,\xi)-\hat{v}(1,\xi)\exp\left(\frac{(1-r)\sin\xi}{\ep   }\right)\chi_{(\pi,2\pi)}\delta(r))C(r,\xi),
% \end{equation}
% where $C(r,\xi)$,$\delta(r)$,$\chi_{(\pi,2\pi)}$ are given by
% (2.18),(2.16) and (2.15) and $\hat{v}(r,\xi) = \hat{u}(x,y)$.
% }

% {\color{gray}
% To compare the performance with EPINN, we used 4 layers for PINN ($\hat{u}$) for square, circular and elliptical domain
% \begin{equation}\label{e:NN}
%     \hat{u}({{x,y}}; \, {\blds \theta})
%     =
%         W_6\sigma(W_5\sigma(W_4\sigma(W_3\sigma(W_1 x+W_2 y+b1)+b2)+b3)+b4),
% \end{equation}
% In case of Time dependent problem, we use
% \begin{equation}\label{e:NN}
%     \hat{u}({{x,y,t}}; \, {\blds \theta})
%     =
%         W_6\sigma(W_5\sigma(W_4\sigma(W_3\sigma(W_1 x+W_2 y+W_t t+b1)+b2)+b3)+b4),
% \end{equation}
% }









% \begin{table}
% {\color{red}
% \begin{tabular}{ |p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|  }
%  \hline
%  \multicolumn{7}{|c|}{Relative $L^2$ error by $L^1$ training (SL-PINN)} \\
%  \hline
%     & square & circle with non compatible & circle with compatible & ellipse 4:1& ellipse 1:4& oscillation\\
%  \hline
%  $\epsilon=10^{-4}$   & $9.5\times10^{-5}$    &$4.2\times10^{-3}$ &  $2.6\times10^{-3}$&  $2.3\times10^{-3}$&  $3.4\times10^{-3}$&  $4.0\times10^{-2}$\\
%  $\epsilon=10^{-6}$&   $1.4\times10^{-4}$  & $3.6\times10^{-3}$   &$4.6\times10^{-3}$ &$5.6\times10^{-3}$&  $4.2\times10^{-3}$&  $5.2\times10^{-2}$\\
%   $\epsilon=10^{-8}$ & $3.9\times10^{-4}$   &$4.3\times10^{-3}$ &$1.8\times10^{-3}$ &  $3.4\times10^{-3}$ &  $4.8\times10^{-3}$ &  $6.2\times10^{-2}$ \\
%  \hline
% \end{tabular}}
% \caption{Comparison table} \label{tab:2}
% \end{table}
% \begin{tabular}{ |p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|  }
%  \hline
%  \multicolumn{7}{|c|}{Relative L2 error by L2 training (EPINN)} \\
%  \hline
%     & square & circle with non compatible & circle with compatible & ellipse 4:1& ellipse 1:4& oscillation\\
%  \hline
%  $\epsilon=10^{-4}$   & $2.5\times10^{-3}$    &$3.2\times10^{-3}$ &  $1.6\times10^{-3}$&  $5.1\times10^{-3}$&  $2.6\times10^{-3}$&  $6.5\times10^{-3}$\\
%  $\epsilon=10^{-6}$&   $2.0\times10^{-3}$  & $2.8\times10^{-3}$   &$1.5\times10^{-3}$ &$3.9\times10^{-3}$&  $1.7\times10^{-3}$&  $7.6\times10^{-3}$\\
%   $\epsilon=10^{-8}$ & $2.0\times10^{-3}$   &$4.7\times10^{-3}$ &$2.3\times10^{-3}$ &  $5.8\times10^{-3}$ &  $2.8\times10^{-3}$ &  $9.5\times10^{-3}$ \\
%  \hline
% \end{tabular}







==> sentences.tex <==



\begin{comment}
Similar work has been referenced in \cite{JUNG201188}, \cite{JT13}, and \cite{Jung2008}.
The following lemmas and theorems apply regardless of whether \(A < B\) or \(A = B\).
\end{comment}

\begin{comment}
Before proceeding, we introduce the formal asymptotic expansion of \( u^\varepsilon \), \( u^\varepsilon \sim \sum_{j=0}^{\infty} \varepsilon^j u^j \), also known as the outer expansion in boundary layer theory. This expansion leads to
\begin{equation}\label{iterative equation}
\left\{
\begin{aligned}
    -u^j_y &= \Delta u^{j-1} & \text{in } D, \\
    u^j &= 0 & \text{on } \Gamma_u.
\end{aligned}
\right.
\end{equation}
Here, for simplicity, we define \( \Delta u^{-1} = f(x, y) \). Solutions \( u^j \) for equation (\ref{iterative equation}) are given by
\begin{equation}\label{iterative solution}
u^j(x, y) = \int_y^{C_u(x)} \Delta u^{j-1}(x, s) \, ds, \quad (x, y) \in D.
\end{equation}
\begin{figure}[htbp]
\centering
\includegraphics[scale=0.4]{fig/coordinate_fig.png}
\caption{The boundary-fitted coordinates \(D^*\) (left) and the domain \(D\) (right)
.} %\label{fig1-1}
\end{figure}
\end{comment}


\begin{comment}
We denote the upper and lower halves of the ellipse by \(C_u(x) = B\sqrt{1 - \frac{x^{2}}{A^{2}}}\) and \(C_l(x) = -B\sqrt{1 - \frac{x^{2}}{A^{2}}}\), respectively. 
\end{comment}
\begin{comment}
    where \( H \) is the metric determinant given by \( H = (a \sinh (R-r) \cos \xi)^2 + (a \cosh (R-r) \sin \xi)^2 \).
\end{comment}


\begin{comment}
We introduce a corrector \(\theta^0\) to adjust boundary values at critical points, deriving equations and establishing solutions using analytical and numerical methods. 
\end{comment}
